The Unified Surface Ricci Flow

Ricci flow deforms the Riemannian metric proportionally to the curvature, such that the curvature evolves according to a heat diffusion process and eventually becomes constant everywhere. Ricci flow has demonstrated its great potential by solving various problems in many fields, which can be hardly handled by alternative methods so far. This work introduces the unified theoretic framework for discrete Surface Ricci Flow, including all common schemes: Thurston's Circle Packing, Tangential Circle Packing, Inversive Distance Circle Packing and Discrete Yamabe. Furthermore, this work also introduces a novel scheme, virtual radius circle packing, under the unified framework. This work gives explicit geometric interpretation to the discrete Ricci energy for all the schemes, and Hessian of the discrete Ricci energy for schemes with Euclidean back ground geometry. The unified frame work deepen our understanding to the the discrete surface Ricci flow theory, and inspired us to discover the new schemes, improved the flexibility and robustness of the algorithms, greatly simplified the implementation and improved the debugging efficiency. Experimental results shows the unified surface Ricci flow algorithms can handle general surfaces with different topologies, and is robust to meshes with different qualities, and effective for solving real problems.

==> Euclidean_CP.tex <==
\subsection{Unified formula for Euclidean Yamabe, inversive distance CP and virtual radius CP}


Given a generalized triangle $\triangle$ and a vertex $v$ of
$\triangle$, the type $\varepsilon$ of $v$ is defined to be $\varepsilon = 1$ if $v$ is in the hyperbolic space, $\varepsilon = 0$ if $v$ in on the infinite boundary and $\varepsilon = -1$ if
$v$ is beyond the infinite boundary. In this way, generalized triangles are classified into ten types $(\varepsilon_1, \varepsilon_2, \varepsilon_3)$,
where $\varepsilon_i\in \{-1, 0, 1\}.$

For Euclidean Yamabe, the triangle has three ideal vertices. Therefore its type is $(0,0,0)$. Its edge lengths are $-u_i,-u_j, \lambda_{ij}$. The length of the horocyclic arc is $l_{ij}$.

For Euclidean inversive distance CP, the triangle has one ideal vertex and two vertices beyond the infinite boundary. Therefore its type is $(0,-1,-1)$. Its edge lengths are $-u_i,-u_j, \lambda_{ij}$. The length of the horocyclic arc is $l_{ij}$.

For Euclidean virtual radius CP, the triangle has one ideal vertex and two vertics in the hyperbolic space. Therefore its type is $(0,1,1)$. Its edge lengths are $-u_i,-u_j, \lambda_{ij}$. The length of the horocyclic arc is $l_{ij}$.

The unified cosine law for the three cases is
$$l^2_{ij}=\frac{e^{\lambda_{ij}}+\varepsilon^2e^{-\lambda_{ij}}-\varepsilon e^{u_i-u_j}-\varepsilon e^{u_j-u_i}}{e^{-u_i}e^{-u_j}},$$
where $\varepsilon=0, 1, -1.$

For Euclidean Yamabe, $\varepsilon=0,$ the above formula becomes
$$l^2_{ij}=\frac{e^{\lambda_{ij}}}{e^{-u_i}e^{-u_j}}=e^{u_i+u_j+\lambda_{ij}}.$$

For Euclidean inversive distance CP, $\varepsilon=-1,$ the above formula becomes
$$l^2_{ij}=\frac{2\cosh{\lambda_{ij}}+e^{u_i-u_j}+e^{u_j-u_i}}{e^{-u_i}e^{-u_j}}.$$
Since $u_i=\ln r_i,$ we have
$$l^2_{ij}=\frac{2\cosh(\lambda_{ij})+r_j r_i^{-1}+ r_i r_j^{-1}}{r_i^{-1}r_j^{-1}}=2\cosh(\lambda_{ij})r_ir_j+r_i^2+r_j^2.$$

For Euclidean virtual radius CP, $\varepsilon=1,$ the above formula becomes
$$l^2_{ij}=\frac{2\cosh{\lambda_{ij}}-e^{u_i-u_j}-e^{u_j-u_i}}{e^{-u_i}e^{-u_j}}.$$
Since $u_i=\ln r_i,$ we have
$$l^2_{ij}=\frac{2\cosh(\lambda_{ij})-r_j r_i^{-1}- r_i r_j^{-1}}{r_i^{-1}r_j^{-1}}=2\cosh(\lambda_{ij})r_ir_j-r_i^2-r_j^2.$$

In fact, this is an indirect approach since we use the cosine law. We can calculate directly using calculus for the three cases.

\begin{figure}[ht!]
\labellist\small\hair 2pt

\endlabellist
%\centering
\includegraphics[scale=0.35]{three}
\caption{}
%\label{}
\end{figure}



\section{Unified Ricci Flow}
\label{sec:new}
There are different approaches to construct discrete surface Ricci flow. In the following we briefly introduce different schemes \cite{Glickenstein_2011}. All of the schemes share the same geometric principles.



\subsection{Thurston's Circle Packing\index{Thurston's circle packing}}
\begin{figure}[h]
\begin{center}
%\includegraphics[width=2.4in]{../figures/unified_ricci_flow/RicciFlow/thurston_circle_packing_configure.eps}&
%\includegraphics[width=2.4in]{../figures/unified_ricci_flow/hyperbolic_tetrahedron/2nd_Thurston_CP_configure.eps}\\
\begin{tabular}{cc}
\includegraphics[width=1.5in]{../figures/Zeng-Fig4.15.a.eps}&
\includegraphics[width=1.25in]{../figures/Zeng-Fig4.15.b.eps}\\
\end{tabular}
\caption{Thurston's circle packing scheme \label{fig:thurston_CP_volume}}
\end{center}
\end{figure}

We associate each vertex $v_i$ with a circle
with radius $r_i$. The conformal factor $u_i = \log r_i$. On edge $[v_i,v_j]$, the two circles intersect
at the angle of $\phi_{ij}$. The edge lengths are
\[
    l_{ij}^2 = r_i^2 + r_j^2 + 2r_i r_j \eta_{ij},
\]
where $\eta_{ij} = \cos \phi_{ij}<1$.
The geometric interpretation of the discrete Ricci energy is as follows. We construct a truncated ideal hyperbolic tetrahedron, the discrete Ricci energy is the volume of the tetrahedron plus a constant. As shown in Fig. \ref{fig:thurston_CP_volume}, we construct a prism in upper half space model of three dimensional hyperbolic space $\mathbb{H}^3$, which is the direct product of the triangle $[v_i,v_j,v_k]$ with the vertical line segment $[0,c]$, where $c>0$ is sufficiently large. Through each vertex circle and the power circle, we construct a hemisphere. Each hemisphere is a hyperbolic plane, which separate $\mathbb{H}^3$ to two half-spaces. The intersection between the prism and all the upper half spaces induced by the hemispheres is the hyperbolic truncated ideal tetrahedron.


\subsection{Tangential Circle Packing\index{tangential circle packing}}
\begin{figure}
\begin{center}
%\includegraphics[width=2.4in]{../figures/unified_ricci_flow/RicciFlow/TangentialCP_configure.eps}&
%\includegraphics[width=2.4in]{../figures/unified_ricci_flow/hyperbolic_tetrahedron/tangential_CP_configure.eps}\\
\begin{tabular}{cc}
\includegraphics[width=1.5in]{../figures/Zeng-Fig4.16.a.eps}&
\includegraphics[width=1.25in]{../figures/Zeng-Fig4.16.b.eps}\\
\end{tabular}
\caption{Tangential circle packing scheme \label{fig:tangential_CP_volume}}
\end{center}
\end{figure}
The circles centered at the vertices are tangential to each other. The edge length is given by
\[
l_{ij}^2 = r_i^2 + r_j^2 + 2r_ir_j \eta_{ij},
\]
where $\eta_{ij}=1$ for all edges. The geometric meaning of the discrete Ricci energy is the volume of hyperbolic truncated ideal tetrahedron up to a constant, as shown in Fig. \ref{fig:tangential_CP_volume}.


\subsection{Inversive Distance Circle Packing\index{inversive distance circle packing}}
%\section{Spherical inversive distance circle packing}



\begin{figure}
\begin{center}
%\includegraphics[width=2.4in]{../figures/unified_ricci_flow/RicciFlow/inversive_distance_configure_angle.eps}&
%\includegraphics[width=2.4in]{../figures/unified_ricci_flow/hyperbolic_tetrahedron/inversive_distance_cp.eps}\\
\begin{tabular}{cc}
\includegraphics[width=1.5in]{../figures/Zeng-Fig4.17.a.eps}&
\includegraphics[width=1.25in]{../figures/Zeng-Fig4.17.b.eps}\\
\end{tabular}
\caption{Inversive distance circle packing scheme\label{fig:inversive_distance_CP_volume}}
\end{center}
\end{figure}
As shown in Fig. \ref{fig:inversive_distance_CP_volume}, the edge length is given by
\[
l_{ij}^2 = r_i^2 + r_j^2 + 2\eta_{ij}r_ir_j,
\]
where $\eta_{ij} > 1$. The discrete Ricci energy is the volume of the hyperbolic truncated tetrahedron up to a constant.


\subsection{Discrete Yamabe Flow\index{discrete Yamabe flow}}
\begin{figure}
\begin{center}
%\includegraphics[width=2.4in]{../figures/unified_ricci_flow/RicciFlow/yamabe_configure_angle.eps}&
%\includegraphics[width=2.4in]{../figures/unified_ricci_flow/hyperbolic_tetrahedron/Yamabe.eps}\\
\begin{tabular}{cc}
\includegraphics[width=1.5in]{../figures/Zeng-Fig4.18.a.eps}&
\includegraphics[width=1.25in]{../figures/Zeng-Fig4.18.b.eps}\\
\end{tabular}
\caption{Discrete Yamabe flow scheme\label{fig:Yamabe_flow_volume}}
\end{center}
\end{figure}
In discrete Yamabe flow scheme, the edge length is given by
\[
l_{ij}^2 = \eta_{ij}r_ir_j = \eta_{ij}e^{u_i}e^{u_j}.
\]
The power circle of $[v_i,v_j,v_k]$ coincides with the circumcircle. In this case, the hyperbolic truncated ideal tetrahedron is constructed as follows. First we construct the prism, then remove the hemisphere induced by the power circle. Then for each vertex $v_i,v_j,v_k$ , we construct a sphere tangent to $v_i$ with (Euclidean) radius $r_i$. Then the tetrahedron is cut off by the spheres. The volume of the resulting tetrahedron is the discrete Ricci energy up to a constant.

\subsection{Virtual Radius Circle Packing\index{virtual radius circle packing}}

\begin{figure}
\begin{center}
%\includegraphics[width=2.4in]{../figures/unified_ricci_flow/RicciFlow/virtual_radius_configure_angle.eps}&
%\includegraphics[width=2.4in]{../figures/unified_ricci_flow/hyperbolic_tetrahedron/virtual_radius_cp.eps}\\
\begin{tabular}{cc}
\includegraphics[width=1.5in]{../figures/Zeng-Fig4.19.a.eps}&
\includegraphics[width=1.25in]{../figures/Zeng-Fig4.19.b.eps}\\
\end{tabular}
\caption{Virtual radius circle packing scheme\label{fig:virtual_radius_CP_volume}}
\end{center}
\end{figure}

The vertex circle radius may be virtual as well, as shown in Fig. \ref{fig:virtual_radius_CP_volume}, where the edge length is given by
\[
l_{ij}^2 = -r_i^2 - r_j^2 + 2\eta_{ij}r_ir_j.
\]
The power circle is construct in the following way. We lift each vertex $v_i,v_j,v_k$ vertically, by the distance $r_i,r_j,r_k$ to get three points in the upper half space. Then through these three points, there exists a unique hemisphere. The intersection of the hemisphere with the plane is the power circle. The hyperbolic truncated ideal tetrahedron is the intersection of the prism and the upper half space induced by the hemisphere. The volume of the hyperbolic truncated ideal tetrahedron is the discrete Ricci energy up to a constant.


==> Euclidean_schemes.tex <==
\section{Geometric Interpretations to Ricci Energies}

The geometric interpretation to Ricci energies of Euclidean and hyperbolic Yamabe schemes were discovered by Springborn, Bobenko in \cite{}. In the current work, we generalize the geometric interpretations to all the schemes covered by the unified framework.


%%In the following, we explain different schemes in details. We only focus on one triangle
%%$[v_i,v_j,v_k]$, with corner angles $\theta_i,\theta_j,\theta_k$, conformal factors $u_i,u_j,u_k$ and edge lengths $l_{ij}$ for edge $[v_i,v_j]$, $l_{jk}$ for $[v_j,v_k]$ and $l_{ki}$ for $[v_k,v_i]$. The Ricci energy of the triangle is
%%\begin{equation}
%%E(u_i,u_j,u_k) = \int^{(u_i,u_j,u_k)} \theta_i du_i + \theta_j du_j +\theta_k du_k.
%%\label{eqn:triangle_ricci_energy}
%%\end{equation}

%Under each background geometry $\mathbb{E}^2$, $\mathbb{H}^2$ and $\mathbb{S}^2$, there are $5$ different schemes: tangential circle packing, Thurston's circle packing, inversive distance circle packing, Yamabe flow and virtual radius circle packing.
%
%\textbf{Different schemes have different advantages and disadvantages. We compare different schemes based on our practical experiences, in terms of the difficulty level for initialization, the conformality of the output, robustness to the low quality triangulations, and the existence of the solution for the given target curvature. The robustness is closely related to the existence of the solution, but not exactly equivalent. It is common that a user-prescribed target curvature has no solution, therefore the Ricci flow will induce degenerated triangles and crash. Sometimes, even the solution exists, the flow path intersects the boundary of the space of all admissible curvatures, then the flow crashes.}
%
%\textbf{Our recent breakthrough in the proof of existence of solutions to Yamabe flow shows that by allowing edge swap to keep the triangulation Delaunay will guarantee the existence of the solution, and greatly improve the robustness. In our future submission, we will explain this in details.}

There are three background geometries: Euclidean $\mathbb{E}^2$, Hyperbolic $\mathbb{H}^2$ and Spherical $\mathbb{S}^2$. Within each background geometry, there are 6 schemes: tangential circle packing, Thurston's circle packing, inversive distance circle packing, Yamabe flow, virtual radius circle packing and the mixed type. In the following, we will explain the geometric interpretation of the Ricci energy of all schemes in details.

The followings are the common principles for constructing the tetrahedron,
\begin{enumerate}
\item The cut sphere for the top vertex is a horosphere for $\mathbb{C}^2$ case, a hyperbolic plane for $\mathbb{H}^2$ case, and a Euclidean sphere for $\mathbb{S}^2$ case.
\item if $\varepsilon_i$ for $v_i$ is $+1,0,-1$, then the cut sphere associated with $v_i$ is a hyperbolic plane (Euclidean hemisphere), a horosphere (Euclidean sphere), or there is no cut sphere associated with $v_i$.
\end{enumerate}


\subsection{Euclidean Background Geometry}

For all schemes with Euclidean background geometry, the geometric interpretation to the discrete Ricci energy in Eqn. \ref{eqn:triangle_ricci_energy} is the volume of a truncated ideal hyperbolic prism. We use the upper half space model for $\mathbb{H}^3$, with Riemannian metric
\[
    ds^2 = \frac{dx^2+dy^2+dz^2}{z^2}
\]
the xy-plane is the infinite plane. We draw the triangle on the xy-plane, and draw vertical lines through three vertices, this gives us a prism. Then we through each vertex circle, we either draw a hyperbolic plane (Euclidean hemispheres orthogonal to the xy-plane) or a horosphere, and/or draw a hyperbolic plane through the power circle. The prism is cut off by these hyperbolic planes or horospheres, the volume of the truncated hyperbolic idea tetrahedron is the discrete Ricci energy in Eqn. \ref{eqn:triangle_ricci_energy}. Details are illustrated by Fig. \ref{fig:cp_schemes}.

In the above construction, the choices of horospheres through one vertex are non-unique. Because we are only interested in the derivative and the Hessian of the energy, different choices will lead to the same result.


%\paragraph{Edge Length} Given a circle packing metric $(\Sigma, \gamma, \eta, \epsilon)$
%The edge length on $[v_i,v_j]$ is given by
%\begin{equation}
%    l_{ij}^2 = 2\eta_{ij} \gamma_i \gamma_j + \epsilon_i \gamma_i^2+ \epsilon_j \gamma_j^2.
%\end{equation}
%where $\epsilon$ is $+1$ for tangential/Thurston's/inversive distance circle packing, $0$ for discrete Yamabe flow, $-1$ for virtual radius circle packing.
%
%\paragraph{Hessian Matrix} The Hessian of the energy function \ref{eqn:triangle_ricci_energy} is the Jacobian
%\begin{equation}
%    \frac{\partial(\theta_i,\theta_j,\theta_k)}{\partial(u_i,u_j,u_k)} = -\frac{1}{2A} L\Theta L^{-1}D,
%\label{eqn:Euclidean_hessain}
%\end{equation}
%In the following, we use the function $s(x) = x$. In the above formula, $A$ is the triangle area
%\begin{equation}
%A = \frac{1}{2} \sin\theta_i s(l_j) s(l_k),
%\label{eqn:A}
%\end{equation}
%the matrix $L$
%\begin{equation}
%L = \left(
%\begin{array}{ccc}
%s(l_i) & 0 & 0 \\
%0 & s(l_j) &0 \\
%0 & 0 & s(l_k)
%\end{array}
%\right)
%\label{eqn:L}
%\end{equation}
%the matrix $\Theta$
%\begin{equation}
%\Theta = \left(
%\begin{array}{ccc}
%-1&\cos \theta_k&\cos \theta_j \\
%\cos \theta_k&-1&\cos \theta_i \\
%\cos\theta_j&\cos \theta_i&-1
%\end{array}
%\right)
%\label{eqn:theta}
%\end{equation}
%and
%\begin{equation}
%D=\left(
%\begin{array}{ccc}
%0& \tau(i,j,k) & \tau(i,k,j) \\
%\tau(j,i,k) &0 & \tau(j,k,i)\\
%\tau(k,i,j) & \tau( k,j,i ) & 0
%\end{array}
%\right)
%\label{eqn:D}
%\end{equation}
%where $\tau(i,j,k) = \frac{1}{2}(l_i^2 + \epsilon_j\gamma_j^2- \epsilon_k\gamma_k^2)$.
%
%The formula for Hessian matrix \ref{eqn:Euclidean_hessain} can be applied for optimizing the Ricci energy using Newton's method.
%
%\paragraph{Geometric Interpretation} The geometric meaning for the Hessian matrix is as follows. As shown in Fig. \ref{fig:cp_schemes}, the \emph{power} of $q$ with respect to $v_i$ is
%\[
%    pow( v_i, q) = | v_i - q |^2 - \epsilon \gamma_i^2.
%\]
%The \emph{power center} $o$ of the triangle satisifies
%\[
%    pow(v_i,o) = pow(v_j,o) = pow(v_k,o).
%\]
%The \emph{power circle} $C$ centered at $o$ with radius $\gamma$, where $\gamma = pow(v_i,o)$. Therefore, for tangential, Thurton's and inversive distance circle packing cases, the power circle is orthogonal to  three circles at the vertices $C_i$, $C_j$ and $C_k$; for Yamabe flow case, the power circle is the circumcircle of the triangle; for virtual radius circle packing, the power circle is the equator of the sphere, which goes through three points $\{v_i + \gamma_i^2 \mathbf{n}, v_j + \gamma_j^2 \mathbf{n}, v_k+\gamma_k^2\mathbf{n}\}$, where $\mathbf{n}$ is the normal to the plane.
%
%Through the power center, we draw line perpendicular to three edges, the perpendicular feets are $w_i,w_j$ and $w_k$ respectively. The distance from the power center to the perpendicular feet are $h_i,h_j$ and $h_k$ respectively. Then it can be shown easily that
%\begin{equation}
%    \frac{\partial \theta_i}{\partial u_j} = \frac{\partial \theta_j}{\partial u_i} = \frac{h_k}{l_k},
%    \frac{\partial \theta_j}{\partial u_k} = \frac{\partial \theta_k}{\partial u_j} = \frac{h_i}{l_i},
%    \frac{\partial \theta_k}{\partial u_i} = \frac{\partial \theta_i}{\partial u_k} = \frac{h_j}{l_j},
%    \label{eqn:geometric_hessian_1}
%\end{equation}
%furthermore,
%\begin{equation}
%\frac{\partial \theta_i}{\partial u_i} = -\frac{h_k}{l_k} - \frac{h_j}{l_j},
%\frac{\partial \theta_j}{\partial u_j} = -\frac{h_k}{l_k} - \frac{h_i}{l_i},
%\frac{\partial \theta_k}{\partial u_k} = -\frac{h_i}{l_i} - \frac{h_j}{l_j}.
%    \label{eqn:geometric_hessian_2}
%\end{equation}
%These two formula induces the formula in Eqn. \ref{eqn:geometric_hessian_0}.



\paragraph{Tangential Circle Packing} Frame (a) in Fig.~\ref{} shows the tangential circle packing scheme, where circles at the end vertices of each edge are tangential to each other. The edge length is the summation of circle radii,
\[
    l_{ij} = \gamma_i + \gamma_j.
\]
The truncated hyperbolic tetrahedron is obtained by cutting off the prism by the hyperbolic planes through all the vertex circles and the power circle.

\paragraph{Thurston's Circle Packing}  As shown in Fig. \ref{fig:cp_schemes} row (b), two circles centered at the end vertices of the same edge intersect each other. Assume the intersection angle on edge $[v_i,v_j]$ is $\phi_{ij}$, where $ \phi_{ij}\in [0,\frac{\pi}{2}]$, which determines the conformal structure coefficient $\eta_{ij}=\cos\phi_{ij}$. Then the edge length is given by
\[
    l_{ij}^2 = 2\cos\phi_{ij} \gamma_i\gamma_j + \gamma_i^2+\gamma_j^2.
\]
The tangential circle packing is the special case of this scheme, where each $\phi_{ij}$ is zero. The construction of the truncated hyperbolic tetrahedron is similar to that of tangent circle packing.

\paragraph{Inversive Distance Circle Packing}  As shown in Fig. \ref{fig:cp_schemes} row (c), this scheme further generalizes Thurston's scheme. On each edge $[v_i,v_j]$, two vertex circles are separated, the discrete conformal structure coefficient $\eta_{ij}>1$. The edge length is given by
\[
    l_{ij}^2 = 2\eta_{ij} \gamma_i\gamma_j + \gamma_i^2+\gamma_j^2.
\]
The construction of the truncated hyperbolic tetrahedron is similar to that for Thurston's circle packing.

\paragraph{Yamabe Flow}  As shown in Fig. \ref{fig:cp_schemes} row (d), the vertex circles shrink to points, the edge length is given by
\[
    l_{ij}^2 = 2\eta_{ij} \gamma_i\gamma_j,
\]
where $\eta_{ij} = \frac{L_{ij}^2}{2}$, $L_{ij}$ is the initial edge length, namely
\[
    l_{ij} = e^{\frac{u_i}{2}} L_{ij} e^{\frac{u_j}{2}}.
\]
The power circle is the circum circle of the triangle. The truncated hyperbolic tetrahedron is constructed as follows: draw a horosphere through the vertices $v_i$,$v_j$ and $v_k$, with Euclidean radii $\gamma_i$, $\gamma_j$ and $\gamma_k$, and draw a hyperbolic plane (a hemisphere) through the power circle. The prism is cut off by these horospheres and the hyperbolic plane.

[Add that the absolute positions of horospheres are unnecessary.]

\begin{figure}
\begin{center}
\vspace{-3cm}
\begin{tabular}{lc}
\includegraphics[width=1.5in]{../figures/scheme/tangent_1.eps}&
\includegraphics[width=3in]{../figures/scheme/tangent.eps}\\
(a) tangential circle packing & $\eta=1$, $\epsilon=1$\\
\includegraphics[width=1.5in]{../figures/scheme/thurston_1.eps}&
\includegraphics[width=3in]{../figures/scheme/thurston_new.eps}\\
(b) Thurston's circle packing & $ 0\le \eta \le 1$, $\epsilon=1$\\
\hspace{-2cm}
\includegraphics[width=2.5in]{../figures/scheme/inverse_2.eps}&
\includegraphics[width=3in]{../figures/scheme/inverse_new.eps}\\
(c) Inversive distance circle packing& $\eta\ge 1$, $\epsilon=1$ \\
\includegraphics[width=1.5in]{../figures/scheme/yamabe_1.eps}&
\includegraphics[width=3in]{../figures/scheme/yamabe_new.eps}\\
(d) Yamabe flow & $\eta>0$, $\epsilon=0$\\
\includegraphics[width=2in]{../figures/scheme/virtual_1.eps}&
\includegraphics[width=3in]{../figures/scheme/virtual_new.eps}\\
(e) virtual radius circle packing & $\eta>0$, $\epsilon=-1$\\
\end{tabular}
\caption{Different circle packing schemes\label{fig:cp_schemes}}
\end{center}
\end{figure}

%\begin{figure}
%\begin{center}
%\begin{tabular}{cc}
%\includegraphics[width=1.5in]{../figures/scheme/tangent_1.eps}&
%\includegraphics[width=4in]{../figures/scheme/tangent.eps}\\
%(a) tangential circle packing & $\eta=1$, $\epsilon=1$\\
%\end{tabular}
%\caption{Different circle packing schemes(a)\label{fig:cp_schemes a}}
%\end{center}
%\end{figure}
%
%\begin{figure}
%\begin{center}
%\begin{tabular}{cc}
%\includegraphics[width=1.5in]{../figures/scheme/thurston_1.eps}&
%\includegraphics[width=4in]{../figures/scheme/thurston.eps}\\
%(b) Thurston's circle packing & $ 0\le \eta \le 1$, $\epsilon=1$\\
%\end{tabular}
%\caption{Different circle packing schemes(b)\label{fig:cp_schemes b}}
%\end{center}
%\end{figure}
%
%\begin{figure}
%\begin{center}
%\begin{tabular}{cc}
%\includegraphics[width=2in]{../figures/scheme/inverse_1.eps}&
%\includegraphics[width=4in]{../figures/scheme/inverse.eps}\\
%(c) Inversive distance circle packing& $\eta\ge 1$, $\epsilon=1$ \\
%\end{tabular}
%\caption{Different circle packing schemes(c)\label{fig:cp_schemes c}}
%\end{center}
%\end{figure}
%
%\begin{figure}
%\begin{center}
%\begin{tabular}{cc}
%\includegraphics[width=2.5in]{../figures/scheme/yamabe_1.eps}&
%\includegraphics[width=4in]{../figures/scheme/yamabe.eps}\\
%(d) Yamabe flow & $\eta>0$, $\epsilon=0$\\
%\end{tabular}
%\caption{Different circle packing schemes(d)\label{fig:cp_schemes d}}
%\end{center}
%\end{figure}
%
%\begin{figure}
%\begin{center}
%\begin{tabular}{cc}
%\includegraphics[width=2in]{../figures/scheme/virtual_1.eps}&
%\includegraphics[width=4in]{../figures/scheme/virtual.eps}\\
%(e) virtual radius circle packing & $\eta>0$, $\epsilon=-1$\\
%\end{tabular}
%\caption{Different circle packing schemes(e)\label{fig:cp_schemes e}}
%\end{center}
%\end{figure}
%
%
%
%
%
%
\begin{figure}
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=2in]{../figures/scheme/mixed_1.eps}&
\includegraphics[width=3in]{../figures/scheme/mixed_new.eps}\\
\end{tabular}
\caption{Mixed type scheme\label{fig:mixed_scheme}}
\end{center}
\end{figure}

\paragraph{Virtual Radius Circle Packing}  As shown in Fig. \ref{fig:cp_schemes} row (e), the vertex circles are with imaginary radius, the edge length is given by
\[
    l_{ij}^2 = 2\eta_{ij}\gamma_i\gamma_j - \gamma_i^2 - \gamma_j^2.
\]
We vertically lift vertex $v_i$ to $p_i$, $p_i = v_i + \gamma_i^2\mathbf{n}$, similarly lift $v_j$ and $v_k$ to $p_j$ and $p_k$. Draw a hemisphere through $p_i$, $p_j$ and $p_k$, orthogonal to the xy-plane. The hemisphere cuts off the prism, the volume of the truncated hyperbolic tetrahedron gives the Ricci energy.


\paragraph{Mixed Scheme} Fig. \ref{fig:mixed_scheme} shows one example of the mixed type scheme, which mixes inversive distance circle packing at $v_i$, virtual radius circle packing $v_j$ and Yamabe flow at $v_k$, namely $(\epsilon_i,\epsilon_j,\epsilon_k)=(+1,-1,0)$. The edge length is given by
\[
l_{k}^2=2\eta_{ij}\gamma_i\gamma_j + \gamma_i^2-\gamma_j^2,l_{i}^2=2\eta_{jk}\gamma_j\gamma_k -\gamma_j^2,l_{j}^2= 2\eta_{ki}\gamma_k\gamma_i + \gamma_i^2.
\]
The power circle is constructed as follows: lift $v_j$ to $p_j=v_j+\gamma_j^2\mathbf{n}$, draw a hemisphere through $v_k$ and $p_j$, and its equator is orthogonal to the circle $(v_i,\gamma_i)$. The Hessian matrix formulae, Eqn. \ref{eqn:geometric_hessian_1} and Eqn. \ref{eqn:geometric_hessian_2}, still hold. We draw hemispheres from the vertex circle $(v_i,\gamma_i)$ and the power circle, and a horosphere through $v_k$ with Euclidean raidus $\gamma_k$, the prims is cut off by these spheres, the volume of the left part is the discrete Ricci energy.


==> experiments.tex <==
\section{Experimental Results}
\label{sec:experiments}


In this section, we report our experimental results based on unified
Ricci flow. We thoroughly compare different schemes in terms of
robustness, conformality, efficiency and initialization difficulty.

\subsection{Experimental Environment}

We implemented the unified Ricci flow algorithms using generic C++
language on Windows platform. The method is based on optimizing the
convex  energy using Newton's method. The sparse linear systems are
solved using Eigen library \cite{eigenweb}. The mesh representation
is based on dynamic halfedge data structure. The current
implementation covers all schemes: tangential circle packing,
Thurston's circle packing, inversive distance circle packing, Yamabe
flow, virtual radius circle packing and mixed type schemes, for
discrete surfaces with Euclidean and hyperbolic background
geometries. The algorithms can handle surfaces different topologies.
The package is accessible for the whole research community.

The computational time is tested on the desktop with 2.00GHz CPU, 3.00G RAM. The geometric data sets are from the public databases, such as \cite{stanford} and \cite{aimatshape}. The human face surfaces were scanned from a high speed and high resolution, phase shifting scanner, as described in \cite{DBLP:journals/ijcv/WangGZWGSH08}. We tested our algorithm on a huge amount of various models, including different sizes and topology types. Some of them are without any refinement or geometric processing, in order to test the robustness of the algorithms. Some of them are re-meshed using the algorithm in \cite{Li13TVCG}.


%\begin{figure}
%\begin{center}
%\begin{tabular}{cccc}
%\includegraphics[width=1.5in]{../figures/alex/alex_tangent_circle.eps}&
%\includegraphics[width=1.5in]{../figures/alex/alex_inversive_circle.eps}&
%\includegraphics[width=1.5in]{../figures/alex/alex_yamabe_circle.eps}&
%\includegraphics[width=1.5in]{../figures/alex/alex_virtual_circle.eps}\\
%\includegraphics[width=1.5in]{../figures/kitten/kitten_tangential.eps}&
%\includegraphics[width=1.5in]{../figures/kitten/kitten_inversive.eps}&
%\includegraphics[width=1.5in]{../figures/kitten/kitten_yamabe.eps}&
%\includegraphics[width=1.5in]{../figures/kitten/kitten_virtual.eps}\\
%Tangential CP & Inversive distance CP&Yamabe flow & Virtual radius CP\\
%\end{tabular}
%\caption{Conformality test for different schemes. on meshes with high quality.\label{fig:alex}}
%\end{center}
%\end{figure}



%\begin{figure}
%\begin{center}
%\begin{tabular}{lc}
%\includegraphics[width=1.5in]{../figures/kitten/kitten_tangential.eps}&
%\includegraphics[width=1.5in]{../figures/kitten/kitten_inversive.eps}\\
%Tangential CP & Inversive distance CP\\
%\includegraphics[width=1.5in]{../figures/kitten/kitten_yamabe.eps}&
%\includegraphics[width=1.5in]{../figures/kitten/kitten_virtual.eps}\\
%Yamabe flow & Virtual radius CP\\
%\end{tabular}
%\caption{Conformality test for different schemes on meshes with low quality.\label{fig:kitten}}
%\end{center}
%\end{figure}

\subsection{Generality Testing}
Fig.~\ref{fig:uniformization_closed_surfaces} and
\ref{fig:uniformization_open_surfaces} demonstrate the generality of
Ricci flow method to handle surfaces with all possible topologies.
Fig. \ref{fig:uniformization_closed_surfaces} shows the
uniformization for closed surfaces, where surfaces are conformally
mapped to the unit sphere, Euclidean plane or the hyperbolic disk.
Fig.~\ref{fig:uniformization_open_surfaces} illustrates the
uniformization for surfaces with boundaries, where compact surface
with boundaries are mapped to constant curvature spaces, such that
all boundaries are mapped to geodesic circles. Suggested by Glickenstein: Although there is not
currently a robust theory of Ricci flow with boundary in the smooth
setting, the discrete Ricci flow can compute the canonical conformal
mapping with high efficacy and efficiency. These two figures cover
all the topology types of compact surfaces.

\begin{figure}
\begin{center}
\begin{tabular}{cccc}
\includegraphics[width=0.2\textwidth]{sophie_original.eps}&
\includegraphics[width=0.2\textwidth]{sophie_modified.eps}\\
(a) low quality face&(b) high quality face\\
\includegraphics[width=0.2\textwidth]{bimba_triangulation.eps}&
\includegraphics[width=0.2\textwidth]{bimba_farmed_triangulation.eps}\\
(c) low quality bimba&(d)high quality bimba
\end{tabular}
\caption{Robustness testing.\label{fig:robust}}
\end{center}
\vspace{-0.6cm}
\end{figure}

The uniformization of the genus zero closed surface can be computed
using Ricci flow with spherical background geometry, or Euclidean
background geometry. The spherical Ricci energy is non-convex,
therefore the spherical Ricci flow is not so stable as the Euclidean
Ricci flow. For surface with multiple boundaries, we used Ricci flow
method with Koebe's iteration \cite{Min2012}.

\subsection{Comparisons Among Schemes}

In the following we compare different schemes of surface Ricci flow
in details.

\paragraph{Robustness}
In practice, the biggest challenge for Ricci flow algorithm is the
robustness. Given a target curvature $\bar{K}$, we need to ensure
the following two points:
\begin{enumerate}
\item The target curvature is admissible, namely, the solution to
the Ricci flow Eqn.~\ref{eqn:discrete_ricci_flow} exists.
\item The solution is reachable. It is possible that the flow hits
the boundary of the admissible curvature space before it hits the
target curvature.
\end{enumerate}
For Tangential circle packing, Thurston's circle
packing, there are theorems describing the admissible curvature
spaces \cite{Thurston97} and \cite{chow_luo_03}. For Euclidean (or
hyperbolic) Yamabe flow, if the Delaunay condition is preserved
during the flow by edge swapping, the admissible curvature space is
given in the recent works \cite{Gu_Luo_Sun_Wu_13} and
\cite{Gu_Guo_Luo_Sun_Wu_14}.



We test robustness to the mesh qualities of different schemes. As
shown in Fig. \ref{fig:robust}, the low quality meshes are
simplified from the raw data, they have many obtuse angles and
degenerated triangles; the high quality meshes are obtained using
the method in \cite{Li13TVCG}. We use different schemes to compute
Riemann mappings. For surfaces with high mesh qualities, all schemes
succeed with comparable running time. For surfaces with low mesh
qualities, tangential circle packing outperforms all other schemes.
The other schemes either crash in the flow process, or pass through
with carefully chosen small step length, therefore, the running
times are much longer.

If we allow the connectivity to be modified during the flow, to
preserve the power Delaunay condition, then all schemes succeed on
both surfaces. This shows the preserving the power Delaunay
condition greatly improves the robustness of the Ricci flow
algorithms.

%We also tested numerical stability of different schemes. In general,
%schemes with hyperbolic background geometry are stabler than those
%with Euclidean background geometry.


\begin{figure}
\begin{center}
\begin{tabular}{cccc}
\includegraphics[width=0.2\textwidth]{alex_tangent_circle.eps}&
\includegraphics[width=0.2\textwidth]{alex_tangent.conformal_angle_ratio.eps}\\
\includegraphics[width=0.2\textwidth]{kitten_tangential.eps}&
\includegraphics[width=0.2\textwidth]{kitten_tangent.conformal_angle_ratio.eps}\\
Tangential CP\\
\includegraphics[width=0.2\textwidth]{alex_inversive_circle.eps}&
\includegraphics[width=0.2\textwidth]{alex_idrf.conformmal_angle_ratio.eps}\\
\includegraphics[width=0.2\textwidth]{kitten_inversive.eps}&
\includegraphics[width=0.2\textwidth]{kitten_idrf.conformal_angle_ratio.eps}\\
Inversive distance CP\\
\includegraphics[width=0.2\textwidth]{alex_yamabe_circle.eps}&
\includegraphics[width=0.2\textwidth]{alex_yamabe.conformal_angle_ratio.eps}\\
\includegraphics[width=0.2\textwidth]{kitten_yamabe.eps}&
\includegraphics[width=0.2\textwidth]{kitten_yamabe.conformal_angle_ratio.eps}\\
Yamabe flow\\
\includegraphics[width=0.2\textwidth]{alex_virtual_circle.eps}&
\includegraphics[width=0.2\textwidth]{alex_virtual.conformal_angle_ratio.eps}\\
\includegraphics[width=0.2\textwidth]{kitten_virtual.eps}&
\includegraphics[width=0.2\textwidth]{kitten_virtual.conformal_angle_ratio.eps}\\
Virtual radius CP\\
\end{tabular}
\caption{Conformality test for different schemes. The face model is
with high mesh quality, the kitten model is with lower mesh quality.
\label{fig:conformality_test}}
\end{center}
\end{figure}

\paragraph{Conformality}
Fig.~\ref{fig:conformality_test} compares the qualities of different
schemes: tangential circle packing, inversive distance circle
packing, Yamabe flow and virtual radius circle packing. The
parameterization is denoted as $\varphi: M\rightarrow\mathbb{R}^2$. We calculate each corner angle in the mesh
before and after the discrete conformal mapping. Then we compute the ratio between two angle values,
take the logarithm. The histogram of the logarithm of the angle ratios is a good measurement for the quality of the discrete conformal mapping. If the mapping has high conformality, then all angle ratios are close to $1$, and the histogram is a delta function at $0$. Otherwise, the histogram is with high standard deviation. From
the histograms in Fig.~\ref{fig:conformality_test}, we can see the
tangential circle packing produces mappings with lower conformity.
The other three schemes produce mappings with similar conformality.

\paragraph{Convergence Rate}
Fig.~\ref{fig:convergence} and table~\ref{tab:convergence} show one
experiment for comparing the convergence rates of different schemes
on four different genus one surfaces. In the experiment, the
curvature error threshold is set to $1e-6$ the step length in
Newton's method is chosen to be $5e-1$. In the
table~\ref{tab:convergence}, each item shows the running time in
seconds, and iterations in the optimization. From the table, we can
see the running time and iterations of different schemes are
similar.

In practice, tangential circle packing is more robust to lower
quality mesh qualities, the step length can be chosen to be larger,
therefore, it converges faster than other schemes.

%\begin{figure}
%\begin{center}
%\begin{tabular}{cccc}
%\includegraphics[width=0.15\textwidth]{../figures/timing/kitten.eps}&
%\includegraphics[width=0.15\textwidth]{../figures/timing/elk.eps}\\
%\includegraphics[width=0.15\textwidth]{../figures/timing/rocker.eps}&
%\includegraphics[width=0.15\textwidth]{../figures/timing/knot.eps}\\
%\end{tabular}
%\caption{Convergence testing.\label{fig:convergence}}
%\end{center}
%\vspace{-0.8cm}
%\end{figure}
%
%\begin{center}
%\hspace{-2cm}
% \begin{table}
%{\tiny \begin{tabular}{|l|l|l|l|l|l|}
%\hline
%mesh & V/F/E & Tan. CP & Inv. Dist. CP & Yamabe Flow & Vir. Rad. CP\\
%\hline
%\hline
%Knot & 9792/19584/29376 & 2.324/18 & 2.314/17 & 2.223/17 & 2.234/17\\
%\hline
%Elk  & 9000/18000/27000 & 3.476/24 & 2.775/28 & 2.938/21 & 2.737/20 \\
%\hline
%Rocker & 10044/20088/30132 & 3.424/23 & 2.891/21 & 2.938/21 & 2.922/21\\
%\hline
%Kitten & 10219/20438/30657 & 4.298/23 & 3.941/21 & 3.933/21 & 3.896/21 \\
%\hline
%\end{tabular}}
%\caption{Convergence test. \label{tab:convergence}}
%\vspace{-0.5cm}
%\end{table}
%\end{center}
\paragraph{Initialization}

In practice, the discrete surfaces are given as triangular meshes,
in the initialization stage, we need to convert the edge length
function to circle packing metric $(\Sigma, \gamma, \eta,
\epsilon)$. For different schemes, this conversion has different
level of difficulties.

For tangential circle packing and Yamabe flow, the initializations
are easy and the resulting circle packing metrics are unique. The
initialization is difficult for Thurston's circle packing, which
requires the intersection angles between two vertex circles are
acute, furthermore, the resulting conformal structure coefficient
$\eta: E\to\mathbb{R}$ may not be unique. For inversive distance,
virtual radius and mixed type schemes, the initializations are
relatively easier, but the resulting circle packing metrics may not
be unique.

In theory, the conformal structure coefficient $\eta$
will affect the admissible curvature space \cite{Thurston97} and
\cite{chow_luo_03}. In practice, we haven't found that different
choices of $\eta$'s make differences in terms of conformality or
robustness.
\begin{figure}
\begin{center}
\begin{tabular}{cccc}
\includegraphics[width=0.2\textwidth]{kitten.eps}&
\includegraphics[width=0.2\textwidth]{elk.eps}\\
\includegraphics[width=0.2\textwidth]{rocker.eps}&
\includegraphics[width=0.2\textwidth]{knot.eps}\\
\end{tabular}
\caption{Convergence testing.\label{fig:convergence}}
\end{center}
\end{figure}

\begin{center}
\hspace{-2cm}
 \begin{table}
{\small \begin{tabular}{|l|l|l|l|l|l|}
\hline
mesh & V/F/E & Tan. CP & Inv. Dist. CP & Yamabe Flow & Vir. Rad. CP\\
\hline
\hline
Knot & 9792/19584/29376 & 2.324/18 & 2.314/17 & 2.223/17 & 2.234/17\\
\hline
Elk  & 9000/18000/27000 & 3.476/24 & 2.775/28 & 2.938/21 & 2.737/20 \\
\hline
Rocker & 10044/20088/30132 & 3.424/23 & 2.891/21 & 2.938/21 & 2.922/21\\
\hline
Kitten & 10219/20438/30657 & 4.298/23 & 3.941/21 & 3.933/21 & 3.896/21 \\
\hline
\end{tabular}}
\caption{Convergence test. \label{tab:convergence}}
\end{table}
\end{center}


==> hyperbolic_schemes.tex <==
\subsection{Hyperbolic Background Geometry}

%For discrete surface with hyperbolic background geometry, with the circle packing metric $(\Sigma,\gamma, \eta, \epsilon)$, suppose the conformal structure coefficient $\eta$ is a constant function defined on edges, then for each edge $[v_i,v_j]$, the edge length is given by
%\[
%    \cosh l_{ij}=\frac{4\eta_{ij}e^{u_i+u_j}+(1+\epsilon_i e^{2u_i})(1+\epsilon_j e^{2u_j})}{(1-\epsilon_i e^{2u_i})(1-\epsilon_j e^{2u_j})},
%\]
%where $u_i = \log \tanh \frac{\gamma_i}{2}$ is the discrete conformal factor, $\epsilon$ is $+1$ for tangential/ Thurston's/inversive distance circle packing, $0$ for discrete Yamabe flow and $-1$ for virtual radius circle packing. The Hessian of the energy function or  the Jacobian has similar formula
%\[
%\frac{\partial(\theta_i,\theta_j,\theta_k)}{\partial(u_i,u_j,u_k)} = -\frac{1}{2A} L\Theta L^{-1}D,
%\]
%where $A$ and $L$ is similar to those in Eqn. \ref{eqn:A} and Eqn. \ref{eqn:L} with $s(x)=\sinh x$,  $\Theta$ is the same as in Eqn. \ref{eqn:theta}, and $D$ is similar to that in Eqn. \ref{eqn:D} with
%\[
%\tau(i,j,k) = \cosh l_i \cosh^{\epsilon_j} \gamma_j - \cosh^{\epsilon_k} \gamma_k.
%\]

\paragraph{Inversive Distance Circle Packing} The tangential and Thurston's circle packings can be unified as inversive distance circle packing. In this scheme $\epsilon$ is $+1$, $\eta_{ij}>0$, the length is given by
\[
    \cosh l_{ij}=\eta_{ij}\sinh \gamma_i \sinh \gamma_j+\cosh \gamma_i \cosh \gamma_j.
\]

As shown in Fig. \ref{fig:energy_volume} 1st row and 2nd column, the hyperbolic tetrahedron has four hyperideal vertices, each vertex is cut by a hyperbolic plane, such that the top section is a hyperbolic triangle with lengths $l_{ij}$, $l_{jk}$ and $l_{ki}$, the ``vertical'' edge lengths are $-u_i$, $-u_j$ and $-u_k$ respectively. The bottom lengths are $\lambda_{ij}$, $\lambda_{jk}$ and $\lambda_{ki}$ respectively, where
\begin{equation}
    \cosh \lambda_{ij} = \eta_{ij}.
    \label{eqn:lambda_eta}
\end{equation}
\paragraph{Yamabe Flow}
In this scheme $\epsilon$ is $0$, $\eta_{ij}>0$, The edge length is given by
\[
    \sinh \frac{l_{ij}}{2}=e^{\frac{u_i}{2}}\sinh \frac{L_{ij}}{2}e^{\frac{u_j}{2}},
\]
where $L_{ij}$ is the initial edge length.

As shown in Fig. \ref{fig:energy_volume} 2nd row and 2nd column, the hyperideal tetrahedron has one hyperideal vertex and three ideal vertices. The top hyperideal vertex is cut by a hyperbolic plane, the section is a hyperbolic triangle with edge lengths $l_{ij}, l_{jk}$ and $l_{ki}$. The three ideal vertices are cut by horosphers, such that the ``vertical'' edge lengths are $-u_i$, $-u_j$ and $-u_k$ respectively. Furthermore, the bottom edge lengths are $\lambda_{ij}$, $\lambda_{jk}$ and $\lambda_{ki}$ respectively, where
\[
    \lambda_{ij} = 2 \log \sinh \frac{L_{ij}}{2} = \log 2\eta_{ij}.
\]

\paragraph{Virtual radius Circle Packing}
In this scheme $\epsilon$ is $-1$, $\eta_{ij}>0$, The edge length is given by
\[
    \cosh l_{ij}=\frac{\eta_{ij}\sinh r_i \sinh r_j +1}{\cosh r_i \cosh r_j}.
\]
As shown in Fig. \ref{fig:energy_volume} 3rd row and 2nd column, the hyperbolic tetrahedron has one hyperideal vertex and three vertices inside $\mathbb{H}^3$. The top hyperideal vertex is cut by a hyperbolic plane, the section is a hyperbolic triangle with edge lengths $l_{ij}, l_{jk}$ and $l_{ki}$. The ``vertical'' edge lengths are $-u_i$, $-u_j$ and $-u_k$ respectively. Furthermore, the bottom edge lengths are $\lambda_{ij}$, $\lambda_{jk}$ and $\lambda_{ki}$ respectively, which are given by $\eta_{ij}, \eta_{jk}$ and $\eta_{ki}$ by Eqn.~\ref{eqn:lambda_eta}.

\paragraph{Mixed type Scheme}

Similar to the Euclidean case, there is the mixed type hyperbolic scheme. The energy function relates to a truncated hyperbolic tetrahedron. It top vertex is hyperideal. It three bottom vertices are determined by the types $\epsilon_i,\epsilon_j$ and $\epsilon_k$. If $\epsilon_i$ is $+1$ ($0$ or $-1$), the vertex corresponding to $v_i$ is hyperideal ( ideal or inside $\mathbb{H}^3$ respectively).  The top section is a hyperbolic triangle with edge lengths $l_{ij}, l_{jk}$ and $l_{ki}$. The ``vertical'' edge lengths are $-u_i$, $-u_j$ and $-u_k$ respectively. Furthermore, the bottom edge lengths are $\lambda_{ij}$, $\lambda_{jk}$ and $\lambda_{ki}$ respectively, which are given by $\eta_{ij}, \eta_{jk}$ and $\eta_{ki}$ by Eqn.~\ref{eqn:lambda_eta}.


%The three cases can be unified as
%$$\cosh l_{ij}=\frac{4I_{ij}\sinh r_i \sinh r_j+[(1+\epsilon)\cosh r_i+1-\epsilon][(1+\epsilon)\cosh r_j+1-\epsilon]}
%{[(1-\epsilon)\cosh r_i+1+\epsilon][(1-\epsilon)\cosh r_j+1+\epsilon]},$$
%where $\epsilon=1,0,-1$ for inversive, Yamabe, virtual respectively. When $\epsilon=0,$ $I_{ij}=\frac12 \sinh^2 \frac{L_{ij}}2.$
%
%After changing variable by using $$e^{u_i}=\frac{e^{r_i}-1}{e^{r_i}+1}=\tanh \frac{r_i}2,$$
%we have
%$$\cosh l_{ij}=\frac{4I_{ij}e^{u_i+u_j}+(1+\epsilon e^{2u_i})(1+\epsilon e^{2u_j})}{(1-\epsilon e^{2u_i})(1-\epsilon e^{2u_j})}.$$
%
%
%The energy function is
%$$w(u_1,u_2,u_3)=\int_c^{(u_1,u_2,u_3)}\sum_{i=1}^3\alpha_i d u_i.$$


%\begin{figure}
%\begin{center}
%\begin{tabular}{ccc}
%Inversive Distance CP & Yamabe flow & Virtual Radius CP\\
%\includegraphics[width=0.166\textwidth]{../figures/energy/inversive_distance_euclidean.eps}&
%\includegraphics[width=0.166\textwidth]{../figures/energy/yamabe_euclidean.eps}&
%\includegraphics[width=0.166\textwidth]{../figures/energy/virtual_radius_euclidean.eps}\\
%Euclidean & & \\
%\includegraphics[width=0.166\textwidth]{../figures/energy/inversive_distance_hyperbolic.eps}&
%\includegraphics[width=0.166\textwidth]{../figures/energy/yamabe_hyperbolic.eps}&
%\includegraphics[width=0.166\textwidth]{../figures/energy/virtual_radius_hyperbolic.eps}\\
%Hyperbolic & & \\
%\includegraphics[width=0.166\textwidth]{../figures/energy/inversive_distance_spherical.eps}&
%\includegraphics[width=0.166\textwidth]{../figures/energy/yamabe_spherical.eps}&
%\includegraphics[width=0.166\textwidth]{../figures/energy/virtual_radius_spherical.eps}\\
%Spherical & & \\
%\end{tabular}
%\caption{Different circle packing schemes\label{fig:cp_schemes}}
%\end{center}
%\end{figure}



==> schemes.tex <==
\section{Various Schemes}
In the following, we explain different schemes in details. We only focus on one triangle
$[v_i,v_j,v_k]$, with corner angles $\theta_i,\theta_j,\theta_k$, conformal factors $u_i,u_j,u_k$ and edge lengths $l_{ij}$ for edge $[v_i,v_j]$, $l_{jk}$ for $[v_j,v_k]$ and $l_{ki}$ for $[v_k,v_i]$. The Ricci energy of the triangle is 
\begin{equation}
E(u_i,u_j,u_k) = \int^{(u_i,u_j,u_k)} \theta_i du_i + \theta_j du_j +\theta_k du_k.
\label{eqn:triangle_ricci_energy}
\end{equation}

Under each background geometry $\mathbb{E}^2$, $\mathbb{H}^2$ and $\mathbb{S}^2$, there are $5$ different schemes: tangential circle packing, Thurston's circle packing, inversive distance circle packing, Yamabe flow and virtual radius circle packing. 
\subsection{Euclidean Background Geometry}
\begin{figure}
\begin{center}
\begin{tabular}{lc}
\includegraphics[width=1.5in]{../figures/Zeng-Fig4.18.a.eps}&
\includegraphics[width=1.25in]{../figures/Zeng-Fig4.18.b.eps}\\
(a) tangential circle packing & $\eta=1$, $\epsilon=1$\\
\includegraphics[width=1.5in]{../figures/Zeng-Fig4.17.a.eps}&
\includegraphics[width=1.25in]{../figures/Zeng-Fig4.17.b.eps}\\
(b) Thurston's circle packing & $ 0\le \eta \le 1$, $\epsilon=1$\\
\includegraphics[width=1.5in]{../figures/Zeng-Fig4.19.a.eps}&
\includegraphics[width=1.25in]{../figures/Zeng-Fig4.19.b.eps}\\
(c) Inversive distance circle packing& $\eta\ge 1$, $\epsilon=1$ \\
\includegraphics[width=1.5in]{../figures/Zeng-Fig4.20.a.eps}&
\includegraphics[width=1.25in]{../figures/Zeng-Fig4.20.b.eps}\\
(d) Yamabe flow & $\eta>0$, $\epsilon=0$\\
\includegraphics[width=1.5in]{../figures/Zeng-Fig4.21.a.eps}&
\includegraphics[width=1.25in]{../figures/Zeng-Fig4.21.b.eps}\\
(e) virtual radius circle packing & $\eta>0$, $\epsilon=-1$\\
\end{tabular}
\caption{Different circle packing schemes\label{fig:cp_schemes}}
\end{center}
\end{figure}

\paragraph{Edge Length} Given a circle packing metric $(\Sigma, \gamma, \eta, \epsilon)$
The edge length on $[v_i,v_j]$ is given by
\begin{equation}
    l_{ij}^2 = 2\eta_{ij} \gamma_i \gamma_j + \epsilon (\gamma_i^2+\gamma_j^2).
\end{equation}

\paragraph{Hessian Matrix} The Hessian of the energy function \ref{eqn:triangle_ricci_energy}is the Jacobian
\begin{equation}
    \frac{\partial(\theta_1,\theta_2,\theta_3)}{\partial(u_1,u_2,u_3)} = -\frac{1}{4A} L\Theta L^{-1}D,
\label{eqn:Euclidean_hessain}
\end{equation}
where $A=\frac{1}{2}\sin\theta_i l_jl_k$ is the area of the triangle, $L =diag(l_i,l_j,l_k)$, 
\[
\Theta = \left(
\begin{array}{ccc}
-1&\cos \alpha_k&\cos \alpha_j \\
\cos \alpha_k&-1&\cos \alpha_i \\
\cos\alpha_j&\cos \alpha_i&-1
\end{array}
\right)
\]
and 
\[
D=\left(
\begin{array}{ccc}
0&l_i^2+\epsilon (r_j^2-r_k^2)&l_i^2+\epsilon (r_k^2-r_j^2) \\
l_j^2+\epsilon (r_i^2-r_k^2)&0&l_j^2+\epsilon (r_k^2- r_i^2) \\
l_k^2+\epsilon (r_i^2- r_j^2)&l_k^2+\epsilon (r_j^2- r_i^2)&0
\end{array}
\right)
\]
The formula for Hessian matrix \ref{eqn:Euclidean_hessain} can be applied for optimizing the Ricci energy using Newton's method.

\paragraph{Geometric Interpretation} The geometric meaning for the Hessian matrix is as follows. As shown in figure \ref{fig:cp_schemes}, the \emph{power} of $q$ with respect to $v_i$ is
\[
    pow( v_i, q) = | v_i - q |^2 - \epsilon \gamma_i^2.
\] 
The \emph{power center} $o$ of the triangle satisifies
\[
    pow(v_i,o) = pow(v_j,o) = pow(v_k,o).
\] 
The \emph{power circle} $C$ centered at $o$ with radius $\gamma$, where $\gamma = pow(v_i,o)$. Therefore, for tangential, Thurton's and inversive distance circle packing cases, the power circle is orthogonal to  three circles at the vertices $C_i$, $C_j$ and $C_k$; for Yamabe flow case, the power circle is the circumcircle of the triangle; for virtual radius circle packing, the power circle is the equator of the sphere, which goes through three points $\{v_i + \gamma_i^2 \mathbf{n}, v_j + \gamma_j^2 \mathbf{n}, v_k+\gamma_k^2\mathbf{n}\}$, where $\mathbf{n}$ is the normal to the plane.

Through the power center, we draw line perpendicular to three edges, the perpendicular feets are $w_i,w_j$ and $w_k$ respectively. The distance from the power center to the perpendicular feet are $h_i,h_j$ and $h_k$ respectively. Then it can be shown easily that
\begin{equation}
    \frac{\partial \theta_i}{\partial u_j} = \frac{\partial \theta_j}{\partial u_i} = \frac{h_k}{l_k},
    \frac{\partial \theta_j}{\partial u_k} = \frac{\partial \theta_k}{\partial u_j} = \frac{h_i}{l_i},
    \frac{\partial \theta_k}{\partial u_i} = \frac{\partial \theta_i}{\partial u_k} = \frac{h_j}{l_j},
    \label{eqn:geometric_hessian_1}
\end{equation}
furthermore,
\begin{equation}
\frac{\partial \theta_i}{\partial u_i} = -\frac{h_k}{l_k} - \frac{h_j}{l_j},
\frac{\partial \theta_j}{\partial u_j} = -\frac{h_k}{l_k} - \frac{h_i}{l_i},
\frac{\partial \theta_k}{\partial u_k} = -\frac{h_i}{l_i} - \frac{h_j}{l_j}.
    \label{eqn:geometric_hessian_2}
\end{equation}

The geometric interpreation to the discrete Ricci energy in Eqn. \ref{eqn:triangle_ricci_energy} is the volume of a truncated ideal hyperbolic prism. We use the upper half space model for $\mathbb{H}^3$, with Riemannian metric 
\[
    ds^2 = \frac{dx^2+dy^2+dz^2}{z^2}
\]
the xy-plane is the infinite plane. We draw the triangle on the xy-plane, and draw vertical lines through three vertices, this gives us a prism. Then we through each vertex circle, we either draw a hyperbolic plane (Euclidean hemispheres orthogonal to the xy-plane) or a horosphere, and/or draw a hyperbolic plane through the power circle. The prism is cut off by these hyperbolic planes or horospheres, the volume of the truncated hyperbolic idea tetrahedron is the discrete Ricci energy in Eqn. \ref{eqn:triangle_ricci_energy}. Details are illustrated by Figure \ref{fig:cp_schemes}.

Suppose on the edge $[v_i,v_j]$, the distance from $v_i$ to the perpendicular foot $w_k$ is $d_{ij}$, the distance from $v_j$ to $w_k$ is $d_{ji}$, then $l_{ij} = d_{ij}+d_{ji}$, and 
\[
    \frac{\partial l_{ij}}{\partial u_i} = d_{ij},     \frac{\partial l_{ij}}{\partial u_j} = d_{ji},
\]
furthermore
\[
    d_{ij}^2+d_{jk}^2+d_{ki}^2 = d_{ik}^2+d_{kj}^2+ d_{ji}^2.
\]
\paragraph{Tangential Circle Packing} Figure \ref{fig:cp_schemes} row (a) shows the tangential circle packing scheme, where circles at the end vertices of each edge are tangential to each other.
\[
    l_{ij} = \gamma_i + \gamma_j.
\] 
The truncated hyperbolic tetrahedron is obtained by cutting off the prism by the hyperbolic planes through all the vertex circles and the power circle.

\paragraph{Thurston's Circle Packing}  As shown in Figure \ref{fig:cp_schemes} row (b), two circles centered at the end vertices of the same edge intersect each other. Assume the intersection angle on edge $[v_i,v_j]$ is $\phi_{ij}$, where $ 0\phi_{ij}\in [0,\frac{\pi}{2}]$, which determines the conformal structure coefficient $\eta_{ij}=\cos\phi_{ij}$. Then the edge length is given by
\[
    l_{ij}^2 = 2\cos\phi_{ij} \gamma_i\gamma_j + \gamma_i^2+\gamma_j^2.
\] 
The tangential circle packing is the special case of this scheme, where each $\phi_{ij}$ is zero. The construction of the truncated hyperbolic tetrahedron is similar to that of tangent circle packing.

\paragraph{Inversive Distance Circle Packing}  As shown in Figure \ref{fig:cp_schemes} row (c), this scheme further generalizes Thurston's scheme. On each edge $[v_i,v_j]$, two circles $C_i$ and $C_j$ are separated, the discrete conformal structure coefficient $\eta_{ij}>1$. The edge length is given by
\[
    l_{ij}^2 = 2\eta_{ij} \gamma_i\gamma_j + \gamma_i^2+\gamma_j^2.
\]
The construction of the truncated hyperbolic tetrahedron is similar.

\paragraph{Yamabe Flow}  As shown in Figure \ref{fig:cp_schemes} row (d), the edge length is given by
\[
    l_{ij}^2 = 2\eta_{ij} \gamma_i\gamma_j,
\]
where $\eta_{ij} = \frac{L_{ij}^2}{2}$, $L_{ij}$ is the initial edge length, namely 
\[
    l_{ij} = e^{\frac{u_i}{2}} L_{ij} e^{\frac{u_j}{2}}.
\]
The power circle is the circum circle of the triangle. The truncated hyperbolic tetrahedron is constructed as follows: draw a horosphere through the vertices $v_i$,$v_j$ and $v_k$, with Euclidean radii $\gamma_i$, $\gamma_j$ and $\gamma_k$, and draw a hemisphere through the power circle. The prism is cut off by these horospheres and the hyperbolic plane.

\paragraph{Virtual Radius Circle Packing}  As shown in Figure \ref{fig:cp_schemes} row (e), the vertex circles are with imaginary radius, the edge length is given by
\[
    l_{ij}^2 = 2\eta_{ij}\gamma_i\gamma_j - \gamma_i^2 - \gamma_j^2.
\]
We vertically lift vertex $v_i$ to $p_i$, $p_i = v_i + \gamma_i^2\mathbf{n}$, similarly lift $v_j$ and $v_k$ to $p_j$ and $p_k$. Draw a hemisphere through $p_i$, $p_j$ and $p_k$, orthogonal to the xy-plane. The hemisphere cuts off the prism, the volume of the truncated hyperbolic tetrahedron gives the Ricci energy. 

\begin{figure}
\begin{center}
\begin{tabular}{c}
\includegraphics[width=0.40\textwidth]{../figures/Zeng-Fig4.16.eps}
\end{tabular}
\caption{Mixed type scheme\label{fig:mixed_scheme}}
\end{center}
\end{figure}

\paragraph{Mixed Scheme} Figure \ref{fig:mixed_scheme} shows the mixed scheme, which mixes inversive distance circle packing at $v_i$, virtual radius circle packing $v_j$ and Yamabe flow at $v_k$, namely $(\epsilon_i,\epsilon_j,\epsilon_k)=(+1,-1,0)$. The edge length is given by
\[
l_{k}^2=2\eta_{ij}\gamma_i\gamma_j + \gamma_i^2-\gamma_j^2,l_{i}^2=2\eta_{jk}\gamma_j\gamma_k -\gamma_j^2,l_{j}^2= 2\eta_{ki}\gamma_k\gamma_i + \gamma_i^2.
\] 
The power circle is constructed as follows: lift $v_j$ to $p_j=v_j+\gamma_j^2\mathbf{n}$, draw a hemisphere through $v_k$ and $p_j$, and its equator is orthogonal to the circle $(v_i,\gamma_i)$. The Hessian matrix formulae still hold \ref{eqn:geometric_hessian_1,eqn:geometric_hessian_2}. We draw hemispheres from the vertex circle $(v_i,\gamma_i)$ and the power circle, and a horosphere through $v_k$ with Euclidean raidus $\gamma_k$, the prims is cut off by these spheres, the volume of the left part is the discrete Ricci energy. 


==> spherical_schemes.tex <==

\subsection{Spherical background geometry}

%The general principle to obtain formula in spherical geometry, we only need to change $\sinh$ and $\cosh$ in hyperbolic geometry into $\sin$ and $\cos$. Given a circle packing metric $(\Sigma,\gamma, \eta,\epsilon)$ with spherical background geometry, the length of an edge $[v_i,v_j]$ is
%\[
%    \cos l_{ij}=\frac{-4\eta_{ij}e^{u_i+u_j}+(1-\epsilon_i e^{2u_i})(1-\epsilon_j e^{2u_j})}{(1+\epsilon_i e^{2u_i})(1+\epsilon_j e^{2u_j})},
%\]
%where $u_i = \log \tan \frac{\gamma_i}{2}$. The Hessian of the energy or the Jacobian has exactly the same formula as hyperbolic case
%\[
%\frac{\partial(\theta_i,\theta_j,\theta_k)}{\partial(u_i,u_j,u_k)} = -\frac{1}{2A} L\Theta L^{-1}D,
%\]
%where $A$ and $L$ is similar to those in Eqn. \ref{eqn:A} and Eqn. \ref{eqn:L} with $s(x)=\sin x$,  $\Theta$ is the same as in Eqn. \ref{eqn:theta}, and $D$ is similar to that in Eqn. \ref{eqn:D} with
%\[
%\tau(i,j,k) = \cos l_i \cos^{\epsilon_j} \gamma_j - \cos^{\epsilon_k} \gamma_k.
%\]


\paragraph{Inversive Distance Circle Packing} The tangential and Thurston's circle packings can be unified as inversive distance circle packing. In this scheme $\epsilon$ is $+1$, $\eta_{ij}>0$, the length is given by
\[
    \cos l_{ij}=\eta_{ij}\sin \gamma_i \sin \gamma_j+\cos \gamma_i \cos \gamma_j.
\]

As shown in Fig. \ref{fig:energy_volume} 1st row and 3rd column, the top vertex of the hyperbolic tetrahedron is inside $\mathbb{H}^3$, with three corner angles $l_{ij}$, $l_{jk}$ and $l_{ki}$. The other three hyperideal vertices are cut by three hyerbolic planes, such that the ``vertical'' edge lengths are $-u_i$, $-u_j$ and $-u_k$ respectively. The bottom lengths are $\lambda_{ij}$, $\lambda_{jk}$ and $\lambda_{ki}$ respectively, where
\begin{equation}
    \cosh \lambda_{ij} = \eta_{ij}.
    \label{eqn::s2_lambda_et}
\end{equation}

\paragraph{Yamabe Flow}
In this scheme $\epsilon$ is $0$, $\eta_{ij}>0$, The edge length is given by
\[
   \sin \frac{l_{ij}}{2}=e^{\frac{u_i}{2}}\sin \frac{L_{ij}}{2}e^{\frac{u_j}{2}},
\]
where $L_{ij}$ is the initial edge length.


As shown in Fig. \ref{fig:energy_volume} 2nd row and 3rd column, the top vertex of the hyperbolic tetrahedron is inside $\mathbb{H}^3$, with three corner angles $l_{ij}$, $l_{jk}$ and $l_{ki}$. The other three ideal vertices are cut by three horospheres, such that the ``vertical'' edge lengths are $-u_i$, $-u_j$ and $-u_k$ respectively. The bottom lengths are $\lambda_{ij}$, $\lambda_{jk}$ and $\lambda_{ki}$ respectively, which are given by $\eta_{ij}
\[
    \lambda_{ij} = \log 2\eta_{ij}.
\]

\paragraph{Virtual radius Circle Packing}
In this scheme $\epsilon$ is $-1$, $\eta_{ij}>0$, The edge length is given by
\[
    \cos l_{ij}=\frac{\eta_{ij}\sin \gamma_i \sin \gamma_j +1}{\cos \gamma_i \cos \gamma_j}.
\]

As shown in Fig. \ref{fig:energy_volume} 3rd row and 3rd column, the hyperbolic tetrahedron has all four vertices inside $\mathbb{H}^3$. The top vertex is with three corner angles $l_{ij}$, $l_{jk}$ and $l_{ki}$, the ``vertical'' edge lengths are $-u_i$, $-u_j$ and $-u_k$ respectively. The bottom lengths are $\lambda_{ij}$, $\lambda_{jk}$ and $\lambda_{ki}$ respectively, where
\[
    \cosh \lambda_{ij} = \eta_{ij}.
\]

\paragraph{Mixed type scheme}
Similar to $\mathbb{E}^2$ and $\mathbb{H}^2$ cases, there is the mixed type for $\mathbb{S}^2$ case. The energy function relates to a truncated hyperbolic tetrahedron. It top vertex is in $\mathbb{H}^3$. It three bottom vertices are determined by the types $\epsilon_i,\epsilon_j$ and $\epsilon_k$. If $\epsilon_i$ is $-1$ ( $0$ or $+1$ ), the corresponding vertex on the textrhedron is hyperideal, ideal or inside $\mathbb{H}^3$ respectively.  The top vertex is with three corner angles $l_{ij}$, $l_{jk}$ and $l_{ki}$, the ``vertical'' edge lengths are $-u_i$, $-u_j$ and $-u_k$ respectively. The bottom lengths are $\lambda_{ij}$, $\lambda_{jk}$ and $\lambda_{ki}$ respectively, where
\[
    \cosh \lambda_{ij} = \eta_{ij}.
\]



==> theory_bak.tex <==
\section{Theoretic Foundations}
This section briefly introduces elementary theories of conformal
geometry. Conformal geometry is the intersection of many fields in
mathematics. We will recall the most fundamental theories in each
field which are closely related to our computational
methodologies.

We refer readers to the following classical books in each field
for detailed proofs for the theories. A thorough introduction
to topological manifolds can be found in Lee's book \cite{Lee00};
 Differential forms, exterior calculus, Hodge decomposition
 theorems, and de Rham cohomology can be found in Lang's book \cite{Lang95}; Farkas
and Kra's text book on Riemann surfaces is excellent
 \cite{FarkasKra91}; do Carmo's textbook \cite{doCarmo76} on
  differential geometry of curves and surfaces gives a good
  introduction to global differential geometry; Ahlfors' classical
   lecture note \cite{Ahlfors66} on quasiconformal mapping gives
   a good introduction; more advanced quasiconformal
   Teichm\"uller theories can be found in Gardiner and Lakic's
   book \cite{GardinerLakic99}; Schoen and Yau's
lectures on harmonic maps \cite{SchoenYau94} and
differential geometry \cite{SchoenYau94_2} give
thorough explanation on harmonic maps and conformal
 metric deformation; recent developments on Ricci flow
 can be found in \cite{Chow06}.

Any non-orientable surface has a two-fold cover which is
orientable. In the following discussion, by replacing a
non-orientable surface by its orientable double cover,we will
always assume surfaces are orientable.

\subsection{Algebraic Topology}

All oriented compact connected two dimensional topological
manifolds can be classified by their genus $g$ and number of
boundaries $b$. Therefore, we use $(g,b)$ to represent the
topological type of a surface $S$.

Suppose $q$ is a base point in $S$. All the oriented closed curves (loops) in $S$ through $q$ can be classified by homotopy. The
set of all such homotopy classes is the so-called
\emph{fundamental group} of $S$, or \emph{the first homotopy
group}, denoted as $\pi_1(S,q)$. The group structure of
$\pi_1(S,q)$ determines the homotopy type of $S$.

For a genus $g$ closed surface, one can find \emph{canonical
homotopy group generators} $\{a_1,b_1,a_2,b_2,\cdots,a_g,b_g\}$,
such that $a_i\cdot a_j = 0$, $b_i\cdot b_j=0$, $a_i\cdot
b_j=\delta_{ij}$, where the operator $r_1 \cdot r_2$ represents
the algebraic intersection number between the two loops $\gamma_1$
and $\gamma_2$, and $\delta_{ij}$ is the Kronecker symbol.


\begin{thm}[Fundamental Group]\cite[Pro.~6.12, p.136~~Exp.~6.13, p.~137]{Lee00} For genus $g$ closed surface with a
set of canonical basis, the fundamental group is given by
\[
    <a_1,b_1,a_2,b_2, \cdots, a_g, b_g |
    a_1b_1a_1^{-1}b_1^{-1}a_2b_2a_2^{-1}b_2^{-1}\cdots
    a_gb_ga_g^{-1}b_g^{-1}=e>.
\]
\end{thm}

Recall that \it covering map \rm  $p:\tilde{S}\to S$ is defined as
follows. First, the map $p$ is surjective. Second, each point
$q\in S$ has a neighborhood $U$ with its preimage
$p^{-1}(U)=\cup_i \tilde{U}_i$ a disjoint union of open sets
$\tilde{U}_i$ so that the restriction of $p$ on each $\tilde{U}_i$
is a homeomorphism. We call $(\tilde{S},p)$ a \emph{covering
space} of $S$. Homeomorphisms of $\tilde{S}$, $\tau: \tilde{S} \to
\tilde{S}$, are called \emph{deck transformations}, if they
satisfy $p\circ \tau = p$. All the deck transformations form a
group, \emph{covering group}, and denoted as $Deck(\tilde{S})$.

Suppose $\tilde{q}\in \tilde{S}$, $p(\tilde{q}) = q$ and surface
$\tilde{S}$ is connected. The projection map $p: \tilde{S} \to S$
induces a homomorphism between their fundamental groups, $p_*:
\pi_1(\tilde{S},\tilde{q}) \to \pi_1(S,q)$, if
$p_*\pi_1(\tilde{S}, \tilde{q})$ is a normal subgroup of
$\pi_1(S,q)$ then

\begin{thm}[Covering Group Structure] \cite[Thm~11.30,~~Cor.~11.31, p.250]{Lee00}The quotient group of $\pi_1(S)/p_*\pi_1(\tilde{S},\tilde{q})$ is isomorphic to the deck transformation group of
$\tilde{S}$.
\[
    \pi_1(S,q)/p_* \pi_1(\tilde{S},\tilde{q}) \cong Deck(\tilde{S}).
\]
\end{thm}

If a covering space $\tilde{S}$ is simply connected (i.e.
$\pi_1(\tilde{S})=\{e\}$),  then $\tilde{S}$ is called a
\emph{universal covering space} of $S$. For universal covering space
\[
    \pi_1(\pi) \cong Deck(\tilde{S}).
\]
The existence of the universal covering space is
given by the following theorem,
\begin{thm}[Existence of the Universal Covering Space] \cite[Thm.~12.8, p.~262]{Lee00}
Every connected and locally simply
connected topological space (in particular,
every connected manifold) has a universal covering space.
\end{thm}

The concept of universal covering space is essential in
Poincar\'{e}-Klein-Koebe Uniformization theorem
\ref{thm:uniformization}, and the Teichm\"uller space theory
\ref{subset:teichmuller_space}. It plays an important role in
computational algorithms as well.


\subsection{Hodge Decomposition}
The following discussion can be found in \cite{Lang95}. Suppose
$S$ is a smooth surface with a differential atlas such that all
coordinate transitions are diffeomorphisms. The tangent space
$T_pS$ is a two-dimensional vector space. Its dual space $T_p^*S$
is the cotangent space of $S$ at $p$. Suppose $\omega \in T_p^*S$,
then $\omega:T_pS\to\mathbb{R}$ is a linear function defined on
$T_pS$. We call $\omega$  a differential 1-form at $p$. A
differential 1-form on $S$ has the local representation
\[
    \omega(x^1,x^2) = \omega_1(x^1,x^2) dx^1 + \omega_2(x^1,x^2)
     dx^2,
\]
where $\{dx^1,dx^2\}$ are the dual differential 1-forms to
$\{\frac{\partial}{\partial x^1},\frac{\partial}{\partial x^2}\}$.
A differential 2-form is a tensor $\omega: T_pS \times T_pS \to
\mathbb{R}$ which is multi-linear and skew symmetric,
$\omega(\xi^1,\xi_2)=-\omega(\xi_2,\xi_1)$. The \emph{wedge
product} of two 1-forms $\omega_1,\omega_2$ is a 2-form defined by
\[
    \omega_1 \wedge \omega_2(\xi_1,\xi_2) = \omega_1(\xi_1) \omega_2 (\xi_2) - \omega_1(\xi_2) \omega_2(\xi_1).
\]
A 2-form has a local representation
$f(x^1,x^2) dx^1 \wedge dx^2$.
Suppose $f:S\to \mathbb{R}$ is a differential
function (0-form),
then the \emph{exterior derivative} of $f$ is a 1-form
\[
    df = \frac{\partial f}{\partial x^1} dx^1 +
    \frac{\partial f}{\partial x^2} dx^2.
\]
The exterior derivative of a 1-form is a 2-form
\[
    d\omega = d(\omega_1 dx^1 + \omega_2 dx^2) =
    (d\omega_1)\wedge dx^1 + (d\omega_2)\wedge dx^2
\]
The exterior derivative of a 2-form is $0$.

The Stokes' theorem shows the exterior derivative operator
is the dual of boundary operator
\begin{thm}[Stokes' Theorem] \cite[Thm.~2.1, p.~310]{Lang95}
 Let $\sigma$ be a differential $k$-chain with boundary
 $\partial \sigma$. Suppose $\omega$ is a differential $k-1$-form.
 Then
\[
    \int_{\partial \sigma} \omega = \int_\sigma d\omega.
\]
\end{thm}
Let $\Omega^k(S)$ denote all the k-forms on $S$, $k=0,1,2$, $d^k$
be the exterior derivative. The map  $d^k:\Omega^k(S) \to
\Omega^{k+1}(S)$ is a linear operator with the property
\[
    d^k \circ d^{k-1} \equiv 0.
\]
Suppose $\omega\in \Omega^{k}(S)$ is a k-form. If there
 exists a $k-1$ form $\eta \in \Omega^{k-1}(S)$ such that
$\omega = d^{k-1}\eta$, then $\omega$ is called
an \emph{exact form}. If $d^k\omega=0$ then $\omega$ is
 called a \emph{closed form}. Exact forms are closed.
\begin{defn}[de Rham Cohomology Group] Suppose $S$ is a differential manifold, the $k$-th de Rham cohomology group is defined as
\[
    H^k(S) = \mathrm{Ker}~d_{k}/\mathrm{Img}~d_{k-1}.
\]
\end{defn}
Suppose $S$ has a Riemannian metric. Then at each point $p$, we
can locally choose parameterization, such that $\{\frac{\partial
}{\partial x^1},\frac{\partial }{\partial x^2}\}$ form an oriented
orthonormal basis at the tangent space $T_p$. Let $\{dx^1,dx^2\}$
be the dual 1-form basis. The \emph{Hodge star} operator at the
point $p$ is a linear map $\star: \Omega^k(S)\to \Omega^{2-k}(S)$
so that at the point $p$,
\begin{equation}
    \star dx^1 = dx^2, \quad \star dx^2 = -dx^1, \quad \star f = fdx^1\wedge dx^2, \quad \star(fdx^1\wedge dx^2) = f.
    \label{eqn:hodge_star}
\end{equation}
The \emph{co-differential operator} $\delta$ is defined as
\begin{equation}
    \delta =  -\star d \star,
    \label{eqn:co_differential_operator}
\end{equation}
\begin{defn}[Laplace Operator] The laplace operator $\Delta :\Omega^k(S) \to \Omega^k(S)$,
\[
    \Delta = \delta d + d\delta.
\]
\end{defn}
Suppose $\omega \in \Omega^k(S)$. Then $\omega$ is called a
\emph{harmonic k-form} if $\Delta \omega = 0$. All the
$k$-harmonic forms form a group, denoted as
$H_\Delta^K(S,\mathbb{R})$, which is isomorphic to the $k$-th de
Rham cohomology group by the following Hodge decomposition
theorem. Let $E$ be the exact forms $\{d\eta | \eta \in
\Omega^{k-1}(S)\}$ and $E^\star$ be the co-exact forms $\{\star d\eta| \eta
\in \Omega^{k-1}(S)\}$. Then
\begin{thm}[Hodge Decomposition] \cite[Thm.~5.1, p.~280]{Lang95} \label{thm:hodge} For a closed orientable
surface $S$ with a Riemannian metric,  any differential form can
be decomposed as the summation of an exact form, a co-exact form
and a harmonic form, i.e.,
\[
    \Omega^k(S) = E \oplus E^\star \oplus H_\Delta.
\]
\end{thm}

\subsection{Riemann Surface}

Classical textbooks for Riemann surface theory are \cite{Forster91}
and \cite{Jost00}.

Intuitively, a Riemann surface is a topological surface with an
extra structure, which can measure angles, but not the lengths.

\begin{defn}[Holomorphic Function]Suppose a complex function
$f: \mathbb{C}\to\mathbb{C}$, $x+iy \to u(x,y)+iv(x,y)$,
satisfies the \emph{Cauchy-Riemann} equation
\[
\frac{\partial u}{\partial x} = \frac{\partial v}{\partial y},\quad\frac{\partial u}{\partial y} = -\frac{\partial v}{\partial x},
\]
then $f$ is a \emph{holomorphic function}.
\end{defn}
Equivalently, define complex differential operators by
\[
\frac{\partial }{\partial z} =
\frac{1}{2}(\frac{\partial}{\partial x}-i\frac{\partial}{\partial
y}), \quad\frac{\partial }{\partial \bar{z}} =
\frac{1}{2}(\frac{\partial}{\partial x}+i\frac{\partial}{\partial
y}).
\]
Then the Cauchy-Riemann equation is
\[
    \frac{\partial f}{\partial \bar{z}} = 0.
\]
A holomorphic function between planar domains preserves angles.
For a general manifold covered by local coordinate charts, if all
transitions are holomorphic, then angles can still be consistently
 defined and measured.


\begin{figure}[h!]
\begin{center}
\begin{tabular}{c}
\epsfig{file=../figures/manifold/RiemannSurface.eps,height=3cm}\\
\psfrag{UA}{$U_\alpha$}
\end{tabular}
\end{center}
\caption{Manifold and atlas.\label{fig:atlas} }
\end{figure}

\begin{defn}[Conformal Atlas] Suppose $S$ is a topological
surface with an atlas $\mathcal{A}$. If all the coordinate
transitions are holomorphic, then $\mathcal{A}$ is called a
conformal atlas.
\end{defn}
Because all the local coordinate transitions are holomorphic,
 the measurements of angles are independent of the choice of
 coordinates. Therefore angles are well defined on the surface.
 The maximal conformal atlas is a conformal structure,
\begin{defn}[Conformal Structure]
Two conformal atlases are equivalent if their
union is still a conformal atlas. Each equivalence
class of conformal atlases is called a \emph{conformal structure}.
\end{defn}

\begin{defn}[Riemann Surface] A topological surface with a
 conformal structure is called a Riemann surface.
\end{defn}

The groups of different types of differential forms on the Riemann
surface are crucial in designing the computational methodologies.

\begin{defn}[Holomorhic Differential] Let $S$ be a Riemann
surface with a conformal atlas $\mathcal{A}$. A holomorphic 1-form
$\Omega$ in $S$ is a complex valued smooth 1-form so that locally
it can be written as $f(z) dz$ in conformal charts $(U, z)$ where
$f(z)$ is an analytic function.

\end{defn}
Each holomorphic 1-form can be decomposed to two conjugate harmonic differential 1-forms, namely
\[
    \omega = \tau + i \star\tau,
\]
where $\tau$ is a real valued harmonic 1-form and $\star$ is
 the Hodge
star operator. All the holomorphic differentials form a group,
which is isomorphic to the first de Rham cohomology group (in
complex coefficient).

\begin{defn}[Conformal Mapping] Suppose $S_1$ and $S_2$ are
two Riemann surfaces, a mapping $f: S_1 \to S_2$ is called a
conformal mapping (holomorphic mapping), if in the local analytic
 coordinates, it is represented as $w=g(z)$ where $g$ is holomorphic.
\end{defn}

\begin{defn}[Conformal Equivalence] Suppose $S_1$ and $S_2$ are
 two Riemann surfaces. If a mapping $f: S_1 \to S_2$ is
 holomorphic, one to one and onto, then $S_1$ and $S_2$ are
  conformally equivalent.
\end{defn}

A \emph{M\"obius transformation } is given by
\begin{equation}
    \rho(z) = \frac{az+b}{cz+d}, \quad a,b,c,d \in \mathbb{C}, \quad ad-bc=1.
    \label{eqn:mobius}
\end{equation}
All Riemann surfaces can be unified by the following theorem:
\begin{thm}[Poincar\'e-Klein-Koebe Uniformization] \cite[p.206]{FarkasKra91} \label{thm:uniformization}
Every  connected Riemann surface $S$ is conformally equivalent to
$D/G$ with $D$ as one of the three canonical spaces:
\begin{enumerate}
\item Extended complex plane $\mathbb{C}\cup \{\infty\}$; \item
Complex plane $\mathbb{C}$; \item Unit disk $D=\{z\in \mathbb{C} |
|z| < 1\}$
\end{enumerate}
where $G$ is a subgroup of M\"obius transformations that acts
freely discontinuous on $D$.   Furthermore, $G \cong \pi_1(S)$.
\end{thm}



\begin{defn}[Circle Domain] A circle domain in a Riemann
surface is a domain so that the components of the complement of
the domain are closed geodesic disks and points. Here a geodesic
disk in a Riemann surface is a topological disk whose lifts in the
universal cover is a round desk in $\bf E^2$ or $\bf S^2$ or $\bf
H^2$.

\end{defn}

\begin{thm}[He and Schramm] \cite[Thm.~0.1]{HeSchramm93}\label{thm:circle_domain}Let $S$ be an open
Riemann surface with finite genus and at most countably many ends.
 Then there is a closed Riemann surface $\tilde{S}$, such
 that $S$ is conformally homeomorphic to a circle
 domain $\Omega$ in $\tilde{S}$. Moreover, the pair
  $(\tilde{S}, \Omega)$ is unique up to conformal homeomorphisms.
\end{thm}


\subsection{Harmonic Maps}
Recall that if $F: \bf R^2 \to \bf R^2$ is linear so that the
domain and target have inner products $g_1$ and $g_2$, then the
$L^2$ norm $|F|$ of $F$ is defined to be $\sqrt{\sum_{i, j}
a_{ij}^2}$ where $[a_{ij}]_{2 \times 2}$ is a matrix
representation of $F$ in orthonormal bases.  Let
$(S_1,\mathbf{g}_1)$ and $(S_2,\mathbf{g}_2)$ be surfaces with
Riemannian metrics and let $f$ be a $C^1$ map from $S_1$ to $S_2$.
The harmonic energy of $f$ is defined as
\[
    E(f) = \int_{S_1} | D(f)|^2 \omega_1 \wedge \omega_2
\]
where $D(f)$ is the derivative of $f$ and $\omega_1 \wedge
\omega_2$ is the area form $dA$ on $S_1$.


\begin{defn}[Harmonic Map] The critical points of the harmonic energy in the space of maps are called harmonic maps.
\end{defn}

For the 2-sphere in the standard metric, we have,

\begin{thm}[Schoen and Yau] \cite[Cor. p.~12]{SchoenYau94}Harmonic maps between genus zero closed metric surfaces are conformal maps.
\label{thm:harmonic_map}
\end{thm}

If the target surface $S_2$ is isometrically embedded in
$\mathbf{R}^3$ and $f$ is given by $f=(f_1,f_2,f_3)$, then the
harmonic energy has a simpler form
\[
    E(f) = \int_{S_1} \sum_i |\nabla f_i|^2 dA,
\]
where $\nabla f_i$ is the gradient of $f_i$. Harmonic maps
satisfy the following Laplace equation
\[
    \Delta_{\mathbf{g}_1} f_i = 0, i = 1,2,3
\]
where $\Delta_{\mathbf{g}_1}$ is the Laplace-Beltrami operator.

%{\bf Remark} Are you sure the above is right? I can see it is
%correct if $f: S_1 \to R^3$. But we are having the constrains that
%$f$ is in the fixed surface $S_2$. I am not convenced that this is
%the right equation.


A very useful property of harmonic maps is the following. Suppose $S_1$ is a topological disk and $\phi: S_1 \to S_2$ is a harmonic map into a a convex planar
domain $S_2$ so that the restriction of $\phi$ on the boundaries
$\phi_{\partial S_1}:
\partial S_1 \to \partial S_2$ is a homeomorphism. Then $\phi$ is a
diffeomorphism in the interior.

%RM: Do you assume that $S_1$ is homeomorphic to $S_2$ to start
%with? otherwise, this does not seems to be right also.

\subsection{Differential Geometry}
The details for the following discussion can be found in Schoen and
Yau's lectures on differential geometry \cite{SchoenYau94_2}.
\begin{defn}[Isothermal Coordinates] Let $S$ be a smooth
 surface with a Riemannian metric $\mathbf{g}$. Isothermal
  coordinates $(u,v)$ for $\mathbf{g}$ satisfy
\[
    \mathbf{g} = e^{2\lambda(u,v)} (du^2 + dv^2).
\]
\end{defn}
Locally, isothermal coordinates always exist \cite{Chern55}. An atlas with all
local coordinates being isothermal is a conformal atlas. Therefore
a Riemannian metric uniquely determines a conformal structure,
namely
\begin{thm} All oriented metric surfaces are Riemann surfaces.
\end{thm}

%{\it RM: The above was known to Gauss and Riemann. We should not
%attribute to Chern. Gauss was the first person who proved the
%existence of isothermal coordinate.}


The Gaussian curvature of the surface is given by
\begin{equation}
    K(u,v) = -\Delta_\mathbf{g} \lambda,
    \label{eqn:gaussian_curvature}
\end{equation}
where $\Delta_\mathbf{g} = e^{-2\lambda(u,v)}(\frac{\partial^2}{\partial u^2} + \frac{\partial^2}{\partial v^2})$ is the Laplace-Beltrami operator induced by $\mathbf{g}$. Although the Gaussian curvature is intrinsic to the Riemannian metric, the total Gaussian curvature is a topological invariant:
\begin{thm}[Gauss-Bonnet] \cite[p.~274]{doCarmo76}\label{thm:gauss_bonnet}
The total Gaussian curvature of a closed metric surface is
\[
    \int_S K dA = 2\pi \chi(S),
\]
where $\chi(S)$ is the Euler number of the surface.
\end{thm}

Suppose $\mathbf{g}_1$ and $\mathbf{g}_2$ are two Riemannian
 metrics on the smooth surface $S$. If there is a differential
  function $\lambda : S \to \mathbb{R}$, such that
\[
    \mathbf{g}_2 =  e^{2\lambda} \mathbf{g}_1,
\]
then the two metrics are \emph{conformal equivalent}. Let the
Gaussian curvatures of $\mathbf{g}_1$ and $\mathbf{g}_2$ be $K_1$
and $K_2$ respectively. Then
 they satisfy the following \emph{Yamabe equation}
\[
    K_2 = \frac{1}{e^{2\lambda}}( K_1 - \Delta_{\mathbf{g}_1} \lambda ).
\]
Detailed treatment to Yamabe equation can be found in Schoen
and Yau's
\cite{SchoenYau94_2} chapter V: \emph{conformal deformation of scalar curvatures}.

Consider all possible Riemannian metrics on $S$. Each conformal
equivalence class defines a \emph{conformal structure}. Suppose a
mapping $f:(S_1,\mathbf{g}_1) \to (S_2,\mathbf{g}_2)$ is
differentiable. If the pull back metric is conformal to the
original metric $\mathbf{g}_1$
\[
    f^*\mathbf{g}_2 = e^{2\lambda} \mathbf{g}_1,
\]
then $f$ is a \emph{conformal mapping}.

Suppose the metric $\mathbf{g}=(g_{ij})$ in local coordinate.
Hamilton introduced the Ricci flow as
\[
    \frac{dg_{ij}}{dt} = -K g_{ij}.
\]
For surface case, Ricci flow is equivalent to Yamabe flow. During the flow, the Gaussian curvature will evolve according
to a heat diffusion process.
\begin{thm}[Hamilton and Chow] \cite[Thm.~B.1, p.~504]{Chow06}
Suppose $S$ is a closed surface with a Riemannian metric. If the
total area is preserved, the surface Ricci flow will
 converge to a Riemannian metric of constant  Gaussian curvature.
\end{thm}
This gives another approach to prove the Poincar\'{e} uniformization theorem \ref{thm:uniformization}. As shown in Figure \ref{fig:uniformization}, all closed surfaces can be conformally deformed to one of the three canonical spaces: the unit sphere $\mathbb{S}^2$, the plane $\mathbb{E}^2$ or the hyperbolic space $\mathbb{H}^2$.

\begin{figure}[h!]
\begin{center}
\begin{tabular}{ccc}
\epsfig{file=../figures/uniformization/bima.eps,height=3.0cm}&
\epsfig{file=../figures/uniformization/kitten.nf10k.cut.eps,height=3.0cm}&
\epsfig{file=../figures/uniformization/knotty_hi.eps,height=3.0cm}\\
\epsfig{file=../figures/uniformization/bima.sphere.1.eps,height=3.0cm}&
\epsfig{file=../figures/uniformization/kitten_domain_3x9.eps,height=3.0cm}&
\epsfig{file=../figures/uniformization/knotty_canonical_ucs_edge.eps,height=3.0cm}\\
Spherical & Euclidean & Hyperbolic \\
\end{tabular}
\end{center}
\caption{Surface uniformization theorem.\label{fig:uniformization} }
\end{figure}

\subsection{Quasi-Conformal Maps}
\begin{figure}[ht]
\centering
\includegraphics[height=3.5cm]{../figures/beltrami/beltrami_fill.eps}
\caption{Illustration of how Beltrami coefficient $\mu$ measures the
distortion by a quasi-conformal map that is an ellipse with dilation
$K$.} \label{beltramicd}
\end{figure}


%----------------------------------------------------------------------------------------------------
\begin{figure}[ht]
\centering
\begin{tabular}{cccc}
%\includegraphics[height=3.0cm]{../figures/quasi/face.eps}&
\includegraphics[height=3.0cm]{../figures/quasi/face_pos.eps}&
\includegraphics[height=3.0cm]{../figures/quasi/face_nf160k.uv.eps}&
%\includegraphics[height=3.0cm]{../figures/quasi/face.uv.eps}&
\includegraphics[height=3.0cm]{../figures/quasi/face_pos2mu2.pos.eps}&
\includegraphics[height=3.0cm]{../figures/quasi/face_pos2mu2.uv.eps}\\
(a) Conformal &(b) Circle Packing &(c) Quasi-conformal &(d) Circle packing\\
mapping & induced by (a) & mapping & induced by (c)\\
\end{tabular}
\caption{Conformal and quasi-conformal mappings for a topological
disk.\label{fig:quasi_disk}}
\end{figure}
%----------------------------------------------------------------------------------------------------

A generalization of a conformal map is called the
\emph{quasi-conformal} map, which is an orientation-preserving
homeomorphism between Riemann surfaces with bounded conformality
distortion. The latter means that the first order approximation of
the quasi-conformal homeomorphism takes small circles to small
ellipses of bounded eccentricity. In particular, a conformal
homeomorphism is quasi-conformal.


Mathematically, $\phi$ is quasi-conformal provided that it
satisfies Beltrami's equation \ref{eqn:beltrami}. In a local
conformal chart, the Beltrami equation takes the form
\begin{equation}
\frac{\partial \phi}{\partial \bar{z}} = \mu(z) \frac{\partial
\phi}{\partial z}, \label{eqn:beltrami}
\end{equation}
where $\mu$, called the \emph{Beltrami coefficient}, is a complex
valued Lebesgue measurable function satisfying $|\mu|_{\infty}<
1$. The Beltrami coefficient measures the deviation of $\phi$ from
conformality. In particular, the map $\phi$ is conformal at a
point $p$ if and only if $\mu(p) = 0$. In general, $\phi$ maps an
infinitesimal circle to a infinitesimal ellipse. Geometrically,
the Beltrami coefficient $\mu(p)$ codes the direction of the major
axis and the ratio of the major and minor axes of the
infinitesimal ellipses. Specifically, the angle of major axis with
respect to the x-axis is $arg \mu(p)/2$ and the ratio of the major
and minor axes is $1+|\mu(p)|$. The angle between the minor axis
and the x-axis is $(arg \mu(p) -\pi)/2$.  The distortion or
dilation is given by:
\begin{equation}
K = \frac{1+|\mu(p)|}{1-|\mu(p)|}.
\end{equation}
\noindent Thus, the Beltrami coefficient $\mu$ gives us all the
information about the conformality of the map (see Figure
\ref{beltramicd}).

If equation \ref{eqn:beltrami} is defined on the extended complex
plane, (the complex plane plus the point at infinity), Ahlfors
proved the following theorem.

\begin{thm}[The Measurable Riemann Mapping] \cite[Thm.~1, p.~10]{GardinerLakic99}
The equation \ref{eqn:beltrami} gives a one-to-one
correspondence between the set of quasi-conformal
homeomorphisms of $\mathbb{C}\cup\{\infty\}$ that fix the
points $0,1$ and $\infty$ and the set of measurable
 complex-valued functions $\mu$ for which $|\mu|_\infty < 1$
 on $\mathbf{C}$.
\end{thm}

Suppose $\phi: \Omega \to \mathbf{C}$ is a quasi conformal map
with Beltrami coefficient $\mu$ defined on some domain $ \Omega
\subset \mathbf{C}$.  Then  the pullback of the canonical
Euclidean metric $\mathbf{g}_0$ under $\phi$ is the metric given
by:
\begin{equation}
\phi^*(\mathbf{g}_0) = |\frac{\partial \phi}{\partial z}|^2 |dz +
\mu(z) d\overline{z})|^2.
\end{equation}

Figure \ref{fig:quasi_disk} shows the conformal and quasi-conformal
mappings for a topological disk, where the Beltarmi coefficient is
set to be $\mu = z$. From the texture mappings in frames (c) and
(d), we can see the conformality is maintained well around the nose tip
(circles to circles), while it is changed a lot along the boundary area
(circles to quasi-ellipses).

\subsection{Teichm\"uller Space}
\label{subset:teichmuller_space} The details for Teichm\"uller
theory can be found in \cite{ImayoshiTaniguchi92} and
\cite{FletcherMarkovic07}.

Given a smooth closed surface $S$, the set of all the conformal
structures on $S$, modulo conformal mappings, is the \emph{Moduli
space} of $S$.  The moduli space, introduced and studied by
Riemann,  is of fundamental importance for theoretical study on
Riemann surfaces. Riemann proved that the moduli space is a finite
dimensional object. This means two Riemann surfaces can be decided
to be conformally equivalent or not by computing a {\it finite}
set of invariants. However, the moduli space is very complicated
 geometrically and topologically. Teichm\"uller's
major contribution is to consider the universal covering space,
called the \emph{Teichm\"uller space}, of the moduli space.


Here is a brief recall of Teichmuller's idea. Fix the smooth
surface $S$ and let $C$ be a conformal structure on $S$. Thus a
Riemann surface is the pair $(S, C)$. Two Riemann surfaces $(S,
C_1)$ and $(S, C_2)$ are conformally equivalent if there is a
conformal map $\phi: (S, C_1) \to (S, C_2)$. The moduli space of
$S$ is the set of all conformal equivalent classes of Riemann
surfaces, i.e., $\{ [(S, C)] |$ $C$ is a conformal structure\}.
Two Riemann surfaces $(S, C_1)$ and $(S, C_2)$ are Teichm\"uller
equivalent if there is a conformal map $\phi: (S, C_1) \to (S,
C_2)$ so that $\phi$ is homotopic to the identity map in $S$. The
Teichm\"uller space of $S$ is the set of all Teichm\"uller
equivalence classes of Riemann surfaces.

Let $S$ be a Riemann surface of genus $g \geq 1$.  The dimension
of the Teichm\"uller space $T_g$ of $S$ is 2 if $g=1$ and is
$6g-g$ if $g >1$.  For $g>1$, by the uniformization theorem, each
Riemann surface $(S, C)$ has a unique Riemannian metric of
constant Gaussian curvature $-1$ in its conformal class. We call
it the uniformization metric.  A Riemannian metric of curvature
$-1$ is also called a hyperbolic metric.  Thus, the Teichm\"uller
space can be rephrased in terms of hyperbolic metrics on $S$.

Teichm\"uller's main theorem says that the Teichm\"uller space is
homeomorphic to the Euclidean space of dimension $6g-6$ (if
$g>1$). In terms of the hyperbolic geometry, there is the well
known Fenchel-Nielsen (global) coordinate for the Teichm\"uller
space which we will describe below.

Given a smooth surface $S$ of genus $g >1$, let us fix a pants
decomposition of $S$ using $3g-3$ disjoint simple loops
$\{\gamma_1, ..., \gamma_{3g-3}\}$, as shown in Figure \ref{fig:pants} (b). Topologically, we decompose
the surface $S$ into $(2g-2)$ 3-holed spheres which are called
pants, as shown in Figure \ref{fig:pants} (a).  Thus one can recover the topological surface $S$ by taking
these $2g-2$ pants and gluing them along boundaries. For
Teichm\"uller theory, one needs to take $2g-2$ geometric pants and
glue them by isometries. This geometric reconstruction process
produces the so called Fenchel-Nielsen coordinate of the
Teichm\"uller space.

Basic facts from hyperbolic geometry say a hyperbolic metric with
geodesic boundary on a 3-holed sphere (called a hyperbolic pants, as shown in Figure \ref{fig:pants} (a))
is determined up to isometry by the lengths of its boundary ($\{\gamma_i, \gamma_j, \gamma_k\}$).
Furthermore, if  two hyperbolic pants are to be glued
isometrically along boundary components, the gluing map is not
unique. It depends on how much twist one must use to glue. Thus
there is an extra twisting parameter for each gluing boundary. In
summary, given a vector $v=(l_1, t_1, l_2, t_2, ..., l_{3g-3},
t_{3g-3}) \in (\mathbf{R_+} \times \mathbf{R})^{3g-3}$, one can
produce a hyperbolic metric $d$ on $S$ as follows. We use $l_i$'s
to produce hyperbolic pants bounded by $\gamma_j$'s and use $t_i$
to produce the isometric gluing.
 This vector $v$ is called the Fenchel-Nielsen coordinate of the
metric $d$ with respect to the pants-decomposition.
Fenchel-Nielsen proved that each hyperbolic metric on $S$ is
Teichm\"uller equivalent to one of the $d$'s constructed above and
different vectors $v$'s produce different hyperbolic metrics. Thus
the Teichm\"uller space is parameterized by the space
$(\mathbf{R_+} \times \mathbf{R})^{3g-3}$ using the
Fenchel-Nielsen coordinate. Detailed proofs can be found in \cite{ImayoshiTaniguchi92} and
\cite{GardinerLakic99}.

\begin{figure}[t!]
\begin{center}
\begin{tabular}{cc}
\epsfig{file=../figures/pants/pants.eps,height=3.0cm}&
\epsfig{file=../figures/pants/decomposition.eps,height=3.0cm}\\
(a) A pair of pants &(b) Pants decomposition\\
\end{tabular}
\end{center}
\caption{A surface of genus $g$ with a hyperbolic metric is
decomposed to $2g-2$ pairs of pants by cutting along closed
geodesics. The twisting angle and length of each cutting loop give
the Fenchel-Nielsen coordinates in the shape space. }
\label{fig:pants}
\end{figure}




%A canonical way for the pants decomposition on a marked Riemann
%surface is as follows: because the surface is with hyperbolic
%uniformization metric, then there is a unique geodesic in each
%homotopy class. we use $[a,b]$ to represent $aba^{-1}b^{-1}$, the
%geodesics in following homotopy classes decompose the surface into
%$2g-2$ pairs of pants,
%\[
%\{b_1,b_2,\cdots, b_g, \Pi_{k=1}{1}[a_k,b_k], \Pi_{k=1}{2}
%[a_k,b_k],\cdots, \Pi_{k=1}{g}[a_k,b_k],
%b_2^{-1}\Pi_{k=1}{1}[a_k,b_k], b_3^{-1}\Pi_{k=1}{2}[a_k,b_k],
%\cdots, b_{g-1}^{-1}\Pi_{k=1}{g-2}[a_k,b_k] \}
%\]

%The conformal
%structure of the surface is uniquely determined by the lengths
%of boundary components. There are three shortest paths connecting
 %each pair of boundary components, e.g. $\tau_i$ connects
%  $\gamma_j,\gamma_k$. Then
%$\tau_i,\tau_j,\tau_k$ separate $S$ to two congruent hyperbolic
%hexagons with right corner angles. We call $\tau_i,\tau_j,\tau_k$ as
%bisectors.

%Suppose two pairs of hyperbolic pants $P_1$ and $P_2$ are glued
%together along a common boundary $\gamma$. Then we fix $P_1$ and
%rotate $P_2$ along $\gamma$, the rotation angle is called the
%\emph{twisting angle}. If the bisectors attaching to $\gamma$ on
%$P_1$ and those on $P_2$ are aligned, then the twisting angle is
%$0$.

%The conformal structure of the surface is determined by the
%conformal structure of each pair of the hyperbolic pants and their
%gluing pattern. The lengths of the cutting loops, and the twisting
%angles on them gives the Fenchel-Nielsen coordinates of the surface
%in the Teichm\"uller space.  Detailed proofs can be found in
%\cite{ImayoshiTaniguchi92} and \cite{GardinerLakic99}.

